Learning When to Switch: Composing Controllers to Traverse a Sequence of Terrain Artifacts

Legged robots often use separate control policiesthat are highly engineered for traversing difficult terrain suchas stairs, gaps, and steps, where switching between policies isonly possible when the robot is in a region that is commonto adjacent controllers. Deep Reinforcement Learning (DRL)is a promising alternative to hand-crafted control design,though typically requires the full set of test conditions to beknown before training. DRL policies can result in complex(often unrealistic) behaviours that have few or no overlappingregions between adjacent policies, making it difficult to switchbehaviours. In this work we develop multiple DRL policieswith Curriculum Learning (CL), each that can traverse asingle respective terrain condition, while ensuring an overlapbetween policies. We then train a network for each destinationpolicy that estimates the likelihood of successfully switchingfrom any other policy. We evaluate our switching methodon a previously unseen combination of terrain artifacts andshow that it performs better than heuristic methods. Whileour method is trained on individual terrain types, it performscomparably to a Deep Q Network trained on the full set ofterrain conditions. This approach allows the development ofseparate policies in constrained conditions with embedded priorknowledge about each behaviour, that is scalable to any numberof behaviours, and prepares DRL methods for applications inthe real world

==> sections/abstract.tex <==
Legged robots often use separate control policies that are highly engineered for traversing difficult terrain such as stairs, gaps, and steps, where switching between policies is only possible when the robot is in a region that is common to adjacent controllers. Deep Reinforcement Learning (DRL) is a promising alternative to hand-crafted control design, though typically requires the full set of test conditions to be known before training. DRL policies can result in complex (often unrealistic) behaviours that have few or no overlapping regions between adjacent policies, making it difficult to switch behaviours. In this work we develop multiple DRL policies with Curriculum Learning (CL), each that can traverse a single respective terrain condition, while ensuring an overlap between policies. We then train a network for each destination policy that estimates the likelihood of successfully switching from any other policy. We evaluate our switching method on a previously unseen combination of terrain artifacts and show that it performs better than heuristic methods. While our method is trained on individual terrain types, it performs comparably to a Deep Q Network trained on the full set of terrain conditions. This approach allows the development of separate policies in constrained conditions with embedded prior knowledge about each behaviour, that is scalable to any number of behaviours, and prepares DRL methods for applications in the real world.

%Bipedal locomotion is particularly challenging over terrain artifacts such as stairs, gaps, and steps. For a robot to traverse a sequence of these artifacts, several control policies may be required. For real bipedal robots, individual policies are developed in a constrained setting, where switching is permitted only when the robot is in an overlapping region between policies. Deep reinforcement learning (DRL) is an alternative to hand crafted control design for complex environments, though typically requiring the full set of target conditions during training, with resultant policies that have few or no states that are suitable for switching. Our method develops several DRL policies, each that can traverse a single respective terrain condition. We expand the set of states that are stable with each policy, while ensuring common regions are visited. We learn when these regions overlap and increase the probability of successfully switching by estimating when to switch from the current policy to the next. We demonstrate our method on a previously unseen combination of terrain artifacts, performing better than several baselines, and comparably to a deep Q learning network trained on the full set of terrain conditions.

% where access to a complete set of terrain conditions during training may be difficult. Furthermore, policies for high dimensional walking robots typically have a very narrow set of states they operate within. With few or no overlapping states between stable regions of subsequent policies, switching to the next policy is difficult or impossible. Our method develops several DRL policies, each that can traverse a single respective terrain condition. We expand the set of states that are stable with each policy, while ensuring common regions are visited. We learn when these regions overlap and increase the probability of successfully switching by estimating when to switch between policies. We demonstrate our method on a previously unseen combination of terrain artifacts, performing better than several baselines, and comparably to a deep Q learning network that has been trained on the full set of terrain conditions.

% Our approach involves training policies and switch estimators only on the single terrain condition they are solvingEach policy and switch estimators are trained only i demonstrated on an unseen test environment. A key component of our method is that each policy and switching estimator are only trained on a single terrain type, though achieve comparable results with a deep Q learning network that has access to the test conditions during training. 

% Bipedal locomotion is particularly challenging over complex terrain artifacts such as stairs, gaps, and jumps. To traverse a combination of these terrain artifacts, several controllers may be required. Deep reinforcement learning (DRL) is an alternative to hand crafted control design for complex environments, though resultant policies typically have a very narrow set of states they operate within and are stable, with few or no overlapping states between subsequent policies. This makes switching between policies difficult or impossible. We train subpolicies that have a realistic gait on a flat surface, that also specialise in a particular terrain type. This ensures an overlap between the states that are stable for each policy. We then learn when to switch between policies by analysing each terrain artifact separately, without ever training on more than one terrain type. Our method has the advantage of training on a single specified terrain condition such that we can add to the control suite as necessary without retraining any other component. We verify our method with a simulated 3D biped, and demonstrate a high success rate on a previously unseen test world. 

% We show that policy switching relies on a  and show our policy switching estimation is superior to several benchmarks.



% trained to solve for a particular training domain. To combine controllers to work together to cover a collection of these artifacts, controllers must have an overlap in their regions of attraction, and we must know when this overlap occurs to safely switch to the next controller. DRL policies often result in unrealistic behaviours that do not have any such overlap. Our solution is to train subpolicies that can each walk on a flat surface before engaging with a designated artifact type., but are a separate policy for each artifact, ensuring a common set of states  each policy has a common each with the same initial conditions and with the ability to walk robustly on an flat surface before engaging with its designated terrain condition. 

% what:
% Combine walking controllers to traverse complex terrain artifacts.
% \begin{itemize}
%     \item
% \end{itemize}
% How:
% - Expand roa of subpolicies
% - Learn when to switch 
% \begin{itemize}
%     \item 
% \end{itemize}
% Need:
% \begin{itemize}
%     \item 
% \end{itemize}





==> sections/background.tex <==
We consider our task to be a Markov Decision Process (MDP) defined by tuple $\{\mathcal{S},\mathcal{A}, R, \mathcal{P}, \gamma\}$ where $s_t \in \mathcal{S}$, $a_t \in \mathcal{A}$, $r_t \in R$ are state, action and reward observed at time $t$, $\mathcal{P}$ is an unknown transition probability from $s_t$ to $s_{t+1}$ taking $a_t$, and $\gamma$ is a discount factor. We use curriculum learning that uses external forces applied to the robot to guide initial learning. These forces are considered an artifact of the environment, therefore our MDP is evolving with the curriculum. For this reason we choose an on policy DRL algorithm, where we only keep a small replay history, outlined in more detail below.

\subsection{Deep Reinforcement Learning for Continuous Control}

The reinforcement learning goal is to maximise the sum of future rewards $R = \sum_{t=0}^{T}\gamma^tr_t$, where $r_t$ is provided by the environment at time $t$ after taking action $a_t$. For continuous control, actions are sampled from a deep neural network policy $a_t\sim\pi(s_t)$, where $a_t$ is a torque applied to each joint.

We predict the value of being in each state $V(s_t) = r_t + \gamma V(s_{t+1})$, which is an estimate of the sum of future rewards $R$. We calculate an advantage from this prediction $A(s_t) = r_t + \gamma V(s_{t+1}) - V(s_t)$ that provides an estimate of how much better or worse action $a_t$ performed compared to what we expected. 

We update the policy $\pi(a_t|s_t)$ by scaling the log probability of taking action $a_t$ by the advantage $A(s_t)$ according to the loss function: $L(\theta) = \mathbb{E}[-\log\pi_\theta(a|s)A(s)]$, where $\theta$ is the policy weights. Intuitively, if we did better than expected we want to increase the probability of performing that action next time, and if we did worse reduce its probability.

In practice this loss can be noisy, and result in large updates to the policy. Insteasd we use Proximal Policy Optimisation~\cite{schulman_proximal_2017}, which uses a surrogate loss that is clipped, preventing policy updates that are too large. We also use Generalised Advantage Estimation (GAE) as a low variance estimate of $A$~\cite{schulman_high-dimensional_2018}. 

\subsection{Sequential Composition}

Sequential composition is the idea that moving from one state to another may involve executing several controllers in sequence. Conceptually, each controller has a set of states that form a funnel, where a robot in any state in the funnel will flow to a convex set of states known as the goal set. Each controller $\pi_i$ has a goal set
$\mathcal{G}(\pi_i) = \{s_i^*\}$ and a Region of Attraction (RoA) $\mathcal{R}(\pi_i) = \{s_0 \in \mathcal{S} : \lim_{t\to\infty} s(t,s_0) = \mathcal{G}(\pi_i)\}$. $\mathcal{G}(\pi_i)$ is a set of states controller $\pi_i$ was designed to operate within, and $\mathcal{R}(\pi_i)$ is a set of states that will converge to a state in $\mathcal{G}(\pi_i)$. Thus $\mathcal{R}(\pi_i)$ acts as a funnel, moving any state $s_0$ in its set towards a state in $\mathcal{G}(\pi_i)$. Provided there exists an initial state $s_0\in \mathcal{R}(\pi_i)$, a common state in $\mathcal{G}(\pi_i)$ and $\mathcal{R}(\pi_j)$, and a target state $s_T \in \mathcal{G}(\pi_j)$, then $\pi_i$ can prepare $\pi_j$, shown in notation as $\pi_i \succeq \pi_j$, and therefore controllers can be backchained to move a robot through the state from $s_0$ to $s_T$.

% $\Phi_i \succcurlyeq \Phi_j$
% Any state that is in the funnel, and hence will move a system to the goal set of states, is referred to as the region of attraction.



% If we have a set of controllers, and therefore a set of funnels, we can backchain controllers so that for the current state w the region of attraction 

% in such a way that a robot can flow through the state of one controller and into the funnel for the next

% The sequential composition of funnels. The goal point
% of each controller lies within the domain of attraction induced
% by the next-lower controller. Each controller is only active
% outside the domains of lower controllers. The lowest con-
% troller stabilizes the system at the final destination.

% Goal set 


% Region of attraction


% Sequential composition

% \begin{equation} 
%     \R = \sum(\bold{x}_t, \bold{u}_t ) = h(\bold{x}_t, \bold{u}_t ) + g(\bold{x}_t, \bold{u}_t ), 
% \end{equation}

% \subsection{Our System}
% Pic of our RL solution: subpolicies, how they are trained
% Pic of 2D and joint space region of attractions: Map with coloured regions. Funnels overhead that represent joint state regions of attraction, with higher level funnels representing joint state controller for each other controller.

==> sections/discussion.tex <==
% Where it is challenging to access to the full set of conditions during development, walking over complex terrain requires specialist policies to navigate difficult terrain types. In order to successfully transition between policies, we show that learning when to switch can occur in single terrain conditions, leading to a scalable method where any number of policies can be added to the control suite as required. 
We introduce a novel method for estimating when to switch between a set a of pre-trained policies. We show that our method improves the stability of switching compared to heuristic methods, where policies and switch estimators only have access to a single terrain during training. Our method also performs comparable to a DQN trained on test conditions (all terrain types), which may not be possible for real systems. By designing policies separately we are able to refine controllers in a constrained setting, and embed prior knowledge about the the required behaviour. Similar to the human delivery driver, our bipedal agent can traverse several difficult terrain types. By understanding when to switch between behaviours our method can scale to any number of terrain conditions, where methods trained on the test set of terrains require retraining (DQN and end-to-end).

We design our policies with an overlapping Region of Attraction (RoA). However, this may not always be the possible, particularly for specialist policies where the RoA represents a very narrow set of states that do not overlap with a simple walking policy. Future work will look at evoking a setup policy that expands the RoA of a given policy to ensure this overlap exists. A limitation of our method is the assumption that we have a terrain oracle, learning to identify the upcoming terrain type is left for future work. We believe that harnessing the capabilities of DRL and combining controllers in a modular way will allow us to expand the locomotion capabilities of legged robots. 

% \brendan{TODO:}
% \brendan{
% \begin{itemize}
%     \item switch plots
%     \item end to end
%     \item DQN
%     \item q table plot
%     \item results
%     \item subpolicies results
%     \item baseline table
% \end{itemize}
% }




==> sections/introduction.tex <==
Legged robots are useful for traversing various terrain conditions where wheeled platforms fail to operate. Terrains that are easily negotiated by humans, however, can present a difficult control problem in robotics \cite{atkeson2016happened}. Consider a delivery driver who jumps down from the delivery vehicle, takes a large step over a break in the sidewalk and walks up the stairs to reach the receiver’s front door. For a last mile delivery robot, it is difficult to design a single locomotion controller that can handle a set of similar tasks. Humanoid robots often use separate control policies that have been meticulously tuned for a specific condition in a constrained setting. 

%Real bipedal robots require harnesses and treadmills to engineer walking policies. Damage to the robot and surroundings is a real risk.

\begin{figure}[tb!]
\centering
\includegraphics[width=1.0\columnwidth]{images/main_pic.png}
% \caption{We pre-train policies for several artifact types including jumps, gaps and stairs, ensuring an Regions of Attraction (RoA) overlap for each policy. As a new terrain type is detected, we switch policies when the robot is in a state that is in the RoA for the next policy.}
\caption{We design policies for each complex terrain type separately, ensuring common regions of the state between policies. Switching in these common regions results in desirable behaviour from the switched policy. To successfully switch between policies we train a switch estimator for each policy that learns when best to switch. Our method involves training on each artifact type separately, where training on multiple artifact types at once may be unavailable or dangerous.}
\label{fig:main_pic}
\vspace{-3mm}
\end{figure}

For highly dynamic robots such as bipeds, transitioning from one policy to the next may only be possible through a very narrow set of states. Activating a policy when the robot is in an unsuitable configuration for the target policy can result in the robot falling over. We refer to the set of all states from which using a policy will result in a desirable stable behaviour as the Region of Attraction (RoA) of the policy~\cite{burridge_sequential_1999}. A state that is in the RoA for more than one policy presents an opportunity where these policies can be switched such that the agent will eventuate in a stable configuration. A robust policy switching method would reduce robot falls, which is a real problem with humanoid robots \cite{atkeson2016happened,kalyanakrishnan2011learning}.

Deep Reinforcement Learning (DRL) has been shown to be an effective method for developing walking policies~\cite{schulman_proximal_2017,heess_emergence_2017,peng_deeploco_2017}, and eliminates some of the hand engineering that is required by classical controllers. Deep neural networks, however do not provide insight as to where the policies will be stable. Generally, DRL policies train on the domain they are required to operate, either with a single end-to-end policy~\cite{heess_emergence_2017}, or by learning when to switch by interacting with the target environment~\cite{merel_hierarchical_2019}. Developing policies on a real system that requires exposure to a large set of terrain types during training may be difficult. Instead, it is more practical to design separate policies and then determine when to switch. This approach also allows us to embed prior knowledge into controller design (such as a rudimentary walking policy), to improve the learning outcomes of each individual policy~\cite{tidd_guided_2020}.

In this work, we first train individual DRL policies, each capable of traversing a single respective terrain artifact. The RoA of each controller is expanded using curriculum learning, while ensuring there exists a set of states common between policies (RoA overlap). We then train a neural network that estimates the probability of successful switching, given the robot state and target policy. We evaluate our approach on a random sequence of terrain types (an example shown in Fig~\ref{fig:main_pic}). We show that learning to switch is more stable than heuristic methods. We also compare our method to learning approaches trained on the test domain (sequence of terrain artifacts rather than individual artifacts), and show that we have comparable results despite interacting with only one terrain condition at a time.

The contributions of this work are two-fold:
\begin{itemize}
\setlength\itemsep{0pt}
    \item We train DRL policies for each terrain type while expanding the RoA of each policy, and ensuring an overlap between them via Curriculum Learning
    \item We design a policy switching network that estimates when the robot is in the RoA for the next policy by predicting the probability of success switching in the current state
\end{itemize}

The organization of this paper is as follows. After reviewing the relevant literature in Sec~\ref{sec:related_work}, we describe our method in Sec~\ref{sec:method}. We define the problem of interest in Sec~\ref{secsec:problem}, present how we train DRL policies for individual terrain types with curriculum learning in Sec~\ref{secsec:individual} and describe our switch estimator in Sec~\ref{secsec:switching}. We present our results in \ref{sec:experiments}, before concluding with a brief discussion in Sec~\ref{sec:conclusion}.

%A summary of our contribution is thus presented. First, using DRL we train several policies, each that is capable of traversing a single respective terrain artifact. We increase the RoA of each controller, while ensuring there exists a set of states common between policies (RoA overlap). Secondly, we estimate when the robot is in the RoA of the next policy before switching, thus increasing the stability of the switch. We train a neural network switch estimator for each target policy with data collected from the respective terrain type only. Thirdly, we test our system on a collection of terrain types. %We show that our method for estimating when to switch outperforms several comparative switching methods, and performs comparably with a deep Q learning network that has access to all terrain combinations during training. 
%Fig.~\ref{fig:main_pic} highlights the problem we are addressing and our contributions.


% Deep reinforcement learning (DRL) provides a method to develop visuomotor policies for complex terrain types, though usually does not provide any stability guarantees.

% To develop policies for robots that are equally able as a person and as a human are suitable for tasks such as autonomous last mile delivery, where the robot is required to move  . Complex terrains such as stairs, wide gaps and high ledges, can be easily traversed by a human, though present an extremely challenging task for a robot. A robotic last mile delivery system might be expected to traverse several different types of non-flat surfaces to reach the recipient. 

% It would be difficult to design a single controller for a legged robot to be proficient through a similar range of domains~\cite{?}, instead a suite of controllers is needed. For highly dynamic robots such as bipeds, transitioning from one controller to the next may only be possible in a very narrow set of joint configurations, where switching controllers outside of this configuration would result in instability~\cite{?}. We refer to the set of all states from which using a controller will result in stable behaviour from the robot as the region of attraction (RoA) of the controller~\cite{?}. A state that is in the RoA for more than one controller presents a location where these controllers can be switched such that the agent will eventuate in a stable configuration. 


% A principle benefit to our approach is we do not need access to the combination of all terrain types during training, i.e. once we have trained our set of policies and estimators, we can deploy our system on any combination of terrain artifacts. This is often not the case for other DRL methods where the agent is required to train on the test domain. The idea of training on a single terrain type scales to real systems where it may only be possible to refine a controller in a well constrained setting on a single artifact, and more difficult and unsafe to expose the robot to every terrain condition during training. It is also possible to add controllers for new terrain types without retraining any previous policies, a feature that increases the scope of our control suite to any number of terrain types. 




% Complex terrains such as stairs, wide gaps and high ledges, can be easily traversed by a human, though present an extremely challenging task for a robot. During daily duties, a delivery driver might be expected to walk over several different types of non-flat surfaces to reach their destination. The driver may need to jump down from a step in the delivery vehicle, take a large step over a break in the sidewalk, then walk up several stairs to reach the recipients front door. 

% It would be difficult to design a single controller for a legged robot to be proficient through a similar range of domains, instead a suite of controllers is needed. For highly dynamic robots such as bipeds, transitioning from one controller to the next may only be possible in a very narrow set of joint configurations, where switching controllers outside of this configuration would result in instability.

% Controllers that enable a bipedal robot to work on non-flat surfaces require the controller have information about the walking surface, and can be very challenging to create. Deep reinforcement learning (DRL) methods provide an alternative to hand crafted control designs, and allow the development of complex visuomotor policies. However, DRL methods usually result in a policy trained to work well for a specific task. Furthermore, the policies are highly non linear, often unrealistic, and difficult to analyse with analytical methods. Typical DRL policies have a very narrow set of states for which they are stable, with the possibility of having no states common between controllers. The set of states that are stable for a given controller we refer to as the region of attraction (RoA).

% Our contribution is twofold: we first design controllers that are capable of traversing complex terrain artifacts using DRL, while ensuring the robot motions are not only realistic, they share configuration space with each other controller. Secondly we learn when a robot state is in the region of attraction of a subsequent controller, and by switching controllers in this state we increase the stability of the robot. We show that our method for estimating when to switch outperforms several comparative methods for switching. Fig.~\ref{fig:main_pic} highlights the problem we are addressing and our primary contribution.

% % Our approach looks at designing policies that have overlapping regions of attraction, and learns where these policies overlap such that we can switch between policies at the appropriate time. 


% A principle benefit to our approach is we do not need access to the test domain, i.e. once we have trained our policies and estimators, we can deploy our system on any combination of terrain artifacts. This idea scales to real systems where it may only be possible to refine a controller in a well constrained setting on a single artifact, and more difficult and unsafe to expose the robot to every expected terrain condition during training. It is also possible to add controllers for new terrain types without retraining any previous policies, a feature that scales to any number of terrain types. 


% \begin{figure}[tb!]
% \centering
% \subfloat[]{%
% \includegraphics[width=0.75\columnwidth]{images/legs.png}}
% \hfill
% \subfloat[]{%
% \includegraphics[width=0.75\columnwidth]{images/sim2real_plot.png}}\hfill
% \caption{a) Sim to real test platform, a torque controlled hexapod leg. b) Visualising the reality gap.}
% \label{fig:approach}
% \vspace{-3mm}
% \end{figure}

==> sections/method.tex <==

\begin{figure}[tb!]
\vspace{2mm}
\centering
\includegraphics[width=0.95\columnwidth]{images/fig2.png}
\caption{
We pre-train a suite of deep reinforcement learning (DRL) policies for a set of terrain conditions, and for each policy we train a switch estimator. Using the current policy $\pi_i$, and detecting upcoming terrain type $j$, we use the switch estimator output $e_j$ to determine when the robot is in a suitable configuration to safely switch to the next policy $\pi_j$. Each policy $\pi_i$ (where $i \in$ $\{$walk, jump, gaps, stairs$\}$) is a neural network with inputs $s_t=\{$robot state, heightmap$\}$ and outputs $a_t$ that are the torques applied to each joint. Each switch estimator $\mathcal{E}$ is a neural network with inputs $s_t=\{$robot state, heightmap$\}$ and outputs $e_j$, where $e_j \in [0,1)$ indicates that the current state is in the region of attraction (RoA) for $\pi_j$: $s_t \in R(\pi_j)$. Switching to $\pi_j$ is safest when $e_j$ is high.
}
\label{fig:method}
\vspace{-3mm}
\end{figure}

A summary of our method is outlined in Fig.~\ref{fig:method}. For each terrain type $i$, where $i \in$ $\{$walk, jump, gaps, stairs$\}$, we train a neural network policy and a switch estimator. We assume access to an oracle terrain detector to determine the upcoming terrain type, and therefore what the next policy will be. The switch estimator $\mathcal{E}_j$ for the next policy $\pi_j$ is activated once the next terrain type is detected, with output $e_j \in [0,1)$ indicating the confidence level that the robot is in the RoA of the next policy.

% : $s_t = \{$ robot state, heightmap $\} \in \mathcal{R}(\pi_j)$.% We evaluate our method on a combination of terrain types and compare our method to several other methods for switching, as well as DRL methods that have been trained on a combination of terrain types. 


\subsection{Problem definition}
\label{secsec:problem}
The problem we consider is a biped in a 3D environment, with 12 torque controlled actuators using the Pybullet simulator~\cite{coumans_pybullet_2020}. The biped model has a mass of 54kg, and uses an average torque of TODOwhen walking on a flat surface with torque limits of TODO. The task of the biped is to navigate obstacles typically navigated by a human delivery driver, as such the robot must traverse stairs, gaps, and a large step. We consider the state $s_t=[rs_t, I_t]$ to be the robot state $rs_{t}$ and heightmap image $I_t$ at time $t$.

\textbf{Robot state}: $rs_t=[J_t, Jv_t, c_t, c_{t-1}, v_{CoM,t}, \omega_{CoM,t}, \\ \theta_{CoM,t}, \phi_{CoM,t}, h_{CoM,t}]$, where $J_t$ are the joint positions in radians, $Jv_t$ are the joint velocities in rad/s, $c_t$ and $c_{t-1}$ are the current and previous contact information of each foot, respectively (four Boolean contact points per foot, plus one variable for no points in contact), $v_{CoM,t}$ and $\omega_{CoM,t}$ are the linear and angular velocities of the body Centre of Mass (CoM), $\theta_{CoM,t}$ and $\phi_{CoM,t}$ are the pitch and roll angles of the CoM, and $h_{CoM,t}$ is the height of the CoM above the terrain. All angles except joint angles are represented in the world coordinate frame. In total there are $51$ elements to the robot state, which is normalised by subtracting the mean and dividing by the standard deviation for each variable (statistics are collected as an aggregate during training).

\textbf{Heightmap}: Perception is provided in the form of a heightmap that moves with the x,y,z and yaw positions of the robot body. A heightmap is a common perception method used in robotics, usually extracted from range measuring sensors such as depth cameras, laser scanners or stereo cameras~\cite{fankhauser_universal_2016}. Other work in DRL for walking uses perception from state information~\cite{lee_composing_2019}, RGB cameras~\cite{merel_hierarchical_2019}, or a heightmap~\cite{peng_deeploco_2017}. In early experiments, we found that using a heightmap improved policy performance compared to providing the ground truth terrain pose. The height map is scaled from 0 (the CoM of the robot) to 1 (2m below the CoM), and has a resolution of $[60,40]$, with a grid size of $0.025$m. The robot itself does not appear in the heightmap, and is centred with a larger view in front. The effective field of view is $0.9$m in front, $0.6$m behind, and $0.5$m to each side. A depiction of the heightmap is shown in Fig.~\ref{fig:method}.


\subsection{Training Policies for Individual Terrain Types}
\label{secsec:individual}
Our switching method requires policies to have a RoA overlap, and provided this condition is met we can employ policies derived from any method. We choose DRL as our method to populate our set of policies. In this section we first introduce the reinforcement learning problem and the algorithm of choice. We then introduce our reward function, and finally our curriculum learning approach that ensures policies have a RoA overlap. 

\textbf{Deep Reinforcement Learning}: We consider our task to be a Markov Decision Process (MDP) defined by tuple $\{\mathcal{S},\mathcal{A}, R, \mathcal{P}, \gamma\}$ where $s_t \in \mathcal{S}$, $a_t \in \mathcal{A}$, $r_t \in R$ are state, action and reward observed at time $t$, $\mathcal{P}$ is an unknown transition probability from $s_t$ to $s_{t+1}$ taking $a_t$, and $\gamma$ is a discount factor. The reinforcement learning goal is to maximise the sum of future rewards $R = \sum_{t=0}^{T}\gamma^tr_t$, where $r_t$ is provided by the environment at time $t$. For continuous control, actions are sampled from a deep neural network policy $a_t\sim\pi_\theta(s_t)$, where $a_t$ is a torque applied to each joint. We update the weights $\theta$ of the policy using Proximal Policy Optimisation (PPO)~\cite{schulman_proximal_2017}.


% We use Proximal Policy Optimisation (PPO) to update a clipped objective function $L(\theta) = \mathbb{E}[\min(\text{ratio}_t\cdot A_t, \text{clip}((\text{ratio}_t, 1 - \epsilon, 1 + \epsilon)A_t)$, where $\text{ratio}_t=\frac{\pi_{\theta}(a_t|s_t)}{\pi_{\theta_{old}(a_t|s_t)}}$ is how far the current policy is from the policy from the previous update, $A_t$ is the advantage calculated with Generalised Advantage Estimation (GAE)~\cite{schulman_high-dimensional_2018}, and $\epsilon$ is a constant clip factor.
% Details can be found in~\cite{schulman_proximal_2017}.

% We predict the value of being in each state $V(s_t) = r_t + \gamma V(s_{t+1})$, which is an estimate of the sum of future rewards $R$. We calculate an advantage from this prediction $A(s_t) = r_t + \gamma V(s_{t+1}) - V(s_t)$ that provides an estimate of how much better or worse action $a_t$ performed compared to what we expected. 

% We update the policy $\pi(a_t|s_t)$ by scaling the log probability of taking action $a_t$ by the advantage $A(s_t)$ according to the loss function: $L(\theta) = \mathbb{E}[\log\pi_\theta(a|s)A(s)]$, where $\theta$ is the policy weights~\cite{schulman_proximal_2017}. Intuitively, if we did better than expected we want to increase the probability of performing that action next time, and if we did worse, reduce its probability.

% In practice this loss can result in large updates to the policy that can adversely affect training. Instead we use a loss defined by Proximal Policy Optimisation (PPO)~\cite{schulman_proximal_2017}. PPO uses a surrogate loss that is clipped, ensuring policy predictions remain close to the predictions from the previous update. We also apply Generalised Advantage Estimation (GAE) as a low variance estimate of $A$~\cite{schulman_high-dimensional_2018}, leading to a more accurate prediction of $V(s_t)$ and faster convergence.  

% \subsection{Robot Information}

% Remove numbers (put in results).
% \textbf{Reward}: We use the same reward function for each policy. Instead of using motion capture as a reference behaviour~\cite{peng_deepmimic_2018}, we design a simple walking gait target policy, constructed without simulator physics. Every terrain type uses the same target policy, even for the stair, jump, and gap terrains. For our work, a common target policy worked well for all terrain types, however specific target policies might be needed for more complex terrain. Our reward function is defined as:
% \[r_t = goal + pos + vel + base + step + act\]
% where:
% \begin{itemize}[leftmargin=*]
%     \item $goal$ is the error between the current heading velocity and goal heading velocity $= w_{goal}\cdot \exp[-c_{goal}\cdot e_{goal}]$.
%     \item $pos$ is the error between the joint positions and the target joint positions $= w_{pos}\cdot \exp[-c_{pos}\cdot e_{pos}]$.
%     \item $vel$ is the error between the current joint velocities and the target joint velocities (calculated with finite differences as in~\cite{peng_deepmimic_2018}) $= w_{vel}\cdot \exp[-c_{vel}\cdot e_{vel}]$.
%     \item $base$ is the CoM error from a target height, and zero roll and pitch positions $= w_{base}\cdot \exp[-c_{base}\cdot e_{base}]$. 
%     \item $step$ encourages stepping close to the middle of a step when in contact, as well as symmetrical step length ($\text{left}_{step}\approx \text{right}_{step}$ when in contact) $= w_{step}\cdot \exp[-c_{step}\cdot e_{step}]$. 
%     \item $act$ is a penalty for excessive torque for each of the $n$ joints $= w_{act}\sum_n(a_t^2)$. 
% \end{itemize}

% $e$ is the error of each respective element. Parameters $w$ and $c$ are tunable weights, which are fixed for all policies. 

\textbf{Guided Curriculum Learning}: Curriculum learning is a systematic way of increasing the difficulty of a task~\cite{bengio_curriculum_2009}, and results in learning attractive walking gaits quickly~\cite{yu_learning_2018}. In our work, \textbf{Guided Curriculum Learning}~\cite{tidd_guided_2020}, we apply curriculum learning to a sequence of tasks, where each stage is completed before the commencement of the next stage. The difficulty of each curriculum is increased as milestones are reached with average episode reward used as the milestone for all stages: as the robot consistently achieves a threshold reward, the difficulty of the current stage is increased. We employ three stages: increasing terrain difficulty while guided by expert forces, reducing the expert forces, and increasing perturbations. 

The first stage is increasing the terrain difficulty with external guidance from a rudimentary target walking policy. It is in this stage we enforce that all policies start from the same set of initial conditions, thus there exists a set of states that are common between policies (RoA overlap). We apply external forces to stabilise the CoM (similar to~\cite{yu_learning_2018}), and to each joint. Forces applied to each joint are determined from a PD controller tracking the rudimentary target walking policy. Once the respective terrain is at its most difficult setting (maximum stair height, step height, and gap length), all external forces are annealed to zero. The third stage increases the magnitude of perturbations. We found adding strong perturbations early hindered training, while increasing gradually in the last curriculum stage allowed for greater final disturbances and more robust policies. By increasing the perturbations we also increase the RoA of the respective policy, i.e. the set of states the policy can safely operate within is now larger. The full details on our curriculum learning approach, including the reward used for training each policy, can be found in our previous work~\cite{tidd_guided_2020}. 

\begin{figure}[tb!]
\centering
\subfloat[]{%
% \includegraphics[width=0.5\columnwidth]{images/estimator.png}}
\includegraphics[height=0.3\columnwidth]{images/estimator.png}}
\hfill
\subfloat[]{%
\includegraphics[height=0.3\columnwidth]{images/multi_roa.png}}
\hfill
\caption{a) A switch estimator is trained for each policy, with data collected from each terrain type separately. Data points are collected around the switch point and given a label of 1 if the robot reaches the goal state, 0 otherwise. b) Early switching results in successful transitions for some policies (green), whereas switching late is more likely to fail (red).}
\label{fig:estimator}
\vspace{-3mm}
\end{figure}

\subsection{Learning When to Switch}
\label{secsec:switching}
Switching from one policy to another by estimating when a state is in the RoA for the next policy is an idea that stems from the sequential composition framework~\cite{burridge_sequential_1999}. Each policy $\pi_i$ has a goal set $\mathcal{G}(\pi_i) = \{s_i^*\}$ where $s=[rs, I]$, and a Region of Attraction (RoA) $\mathcal{R}(\pi_i) = \{s_0 \in \mathcal{S} : \lim_{t\to\infty} s(t,s_0) = \mathcal{G}(\pi_i)\}$. $\mathcal{G}(\pi_i)$ is the set of states policy $\pi_i$ was designed to operate within (Goal Set or Invariant Set), and $\mathcal{R}(\pi_i)$ is the set of states that will converge to a state in $\mathcal{G}(\pi_i)$. 

The complete set of states of the RoA for a complex biped is difficult to determine. Instead, we estimate when the robot is in the RoA of a given policy by training a neural network switch estimator. We train a switch estimator for each policy. In other words, each policy has its own switch estimator that is activated once its respective target terrain type is detected. If we switch policies when the switch estimator for the upcoming policy predicts a high value, then the likelihood of the robot safely traversing the target terrain is increased.

The data collection procedure for switching is as follows. A sample is collected by running $\pi_j$ on terrain condition $i$ and switching to $\pi_i$ a random distance from the terrain artifact (where $j \neq i$). As shown in Fig.~\ref{fig:estimator}a), there are three steps to data collection that occur for each sample: detection, switching, and labelling. Detection occurs when the terrain artifact appears $0.9$m from the robot body. We switch to the target policy at a distance $\sim\mathcal{U}(0,0.9)$m from the artifact. A total of 5 data points (robot state + heightmap) are collected for each sample, including the data point when switching occurred at timestep $t$ and the surrounding data points: $[t-2, t-1, t, t+1, t+2]$. The sample (all 5 data points) is labelled as successful (1) if the robot is able to traverse the terrain artifact and not fall for two complete steps. Otherwise, all data points in the sample are labelled as failed (0).  

% and remain stable for several meters after the terrain artifact

% reaches the goal zone (0.9m after the artifact) while maintaining a nominal $v_{CoM}$ and $h_{CoM}$ as a result of the switch that occur at time $t$. Otherwise, all the data points in the sample are labelled as failed (0). 
% We assume that the states that have close proximity to each other should have a similar success prediction, allowing us to collect five times more data for each sample, while smoothing the switch estimations.


Each switch estimator $\mathcal{E}_i$ is trained to minimise the loss $L(\phi) = (\mathcal{E}_i(s_t) - y_t)^2$, where $\phi$ is the neural network weights, $s_t$ is the state and $y_t$ is the corresponding label for data point $t$. The final layer of the network is a single output with a sigmoid activation. Data is split into 90\% training and 10\% validation, with a 50/50 split of positive and negative labels forced during training and validation. We collected a total of 100000 data points for each terrain type, and trained each switch estimator for 1500 epochs.





% To ensure RoA overlap, each policy must first stand for a random number of timesteps, then walk on a flat surface. We provide as additional input a velocity command input $v_t$. The velocity command parameter $v_t$ is concatenated with the robot state, which is set to 0 for standing, and 1 when the robot should move. 

% \paragraph{First Stage - Learning to Walk}
% The initial curriculum provides external forces to stabilise the centre of mass of the robot similar to~\cite{yu_learning_2018}. In addition, we provide an expert guided force at each actuator. Using our target walking policy introduced in the reward function section, we apply a target torque to each joint, calculated using a PD gain on the error between the robot joint positions and target joint positions. The target torque is added to the torque output from the policy. Importantly, the additional torque from the target PD controller is not considered in the gradient calculations of the policy, and is instead an artifact of the evolving environment. We found that providing this additional torque allows the robot to visit relevant parts of the state early in training, significantly increasing learning. The external forces, including the PD gain used to calculate the target torques, are annealed to zero before the next curriculum stage. Given each policy can walk on a flat surface after the first stage, an alternative approach could use a base walking policy as an initialisation for each policy. However, as the first stage is typically completed within the first 10\% of training, we simply train each policy from a random initialisation.

% \paragraph{Second Stage - Adapting the Terrain}
% After the first stage of training, each policy is capable of walking on a flat surface with no help from external forces. The terrain is slowly changed in the second stage, adding height to stairs and jumps, and length to gaps. Stairs are randomly selected as up or down. Gaps and jumps are added at random distance intervals with flat terrain otherwise. Each policy evolves to traverse its designated terrain condition, while sharing the same initial conditions. The second stage takes about 50\% of the training time (harder terrains take longer).

% \paragraph{Third Stage - Adding External Perturbations}
% In the final stage, and for the remainder of training, we add a curriculum of external perturbations. Adding random external forces is a way to improve the robustness of a policy~\cite{schulman_proximal_2017}, though too much noise early in training is a detrimental to learning. We apply an impulse force of random magnitude to the centre of mass in all 6 degrees of freedom of the torso. The force is sampled from a uniform distribution with a maximum value that is increased with each milestones. The force is applied for a single timestep (impulse), at random intervals of around 2 Hz. Having a dedicated curriculum for external disturbances allows us to use a large force that would otherwise prevent training if employed earlier. Once the third curriculum stage is complete, the maximum linear impulse force is 500N and the maximum torsional impulse force is 250Nm. In depth details and analysis of our sequential curriculum method is left for another work.




% \begin{figure}[tb!]
% \centering
% \includegraphics[width=1.0\columnwidth]{images/fig2.png}
% \caption{

% We pre-train a suite of policies for a set of terrain conditions, and each policy has a switch estimator. Using the current policy $i$, and detecting upcoming terrain type $j$, we use the switch estimator output $e_j$ to determine when the robot is in a suitable configuration to safely switch to the next policy $j$.

% We train a set of RL policies 
% $\pi_i$ on specific terrains where $i \in \{walk, jump, gaps, stairs\}$. 
% Each policy takes the state $s_t = \{robot state, heightmap\}$, and produces the next action, $a_t^i$ specifying the torques for each joint. Each policy also estimates $e_i \in [0,1)$ that the current state is in the region of attraction for this policy $s_t \in R(\pi_j)$. The upcoming policy $j$ is determined by a an assumed classifier of the terrain. The active policy $i$ is switched to $j$ when $e_j$ indicates the state, is in the region of attraction for the next policy .


% We train a set of RL policies $\pi_i$ on specific terrains where $i \in \{walk, jump, gaps, stairs\}$. Each policy takes the state S= {robot state, height map}, and produces the next action, $\a_i$ specifying the torques for each joint. Each policy also estimates $e_i \in [0,1)$ that the current state is in the region of attraction for this policy $S \ in R(\pi_j)$. The upcoming policy $j$ is determined by a an assumed classifier of the terrain. The active policy $i$ is switched to $j$ when $e_j$ indicates the state, is in the region of attraction for the next policy .

% We pre-train a suite of policies for a set of terrain conditions, and each policy has a switch estimator. Using the current policy $i$, and detecting upcoming terrain type $j$, we use the switch estimator output $e_j$ to determine when the robot is in a suitable configuration to safely switch to the next policy $j$.

% that determines when the robot is in a safe configuration for switching.

% For each policy $i$ we train a switch estimator with output $e_i$ that indicates when the robot is in a safe configuration to policy $i$.

% \caption{We train a set of policies $\pi$, and a switch estimator for each policy $\mathcal{R}(\pi)$. Each policy and switch estimator is trained on a single terrain artifact, we then evaluate our system in a test world with all artifact types. As the robot detects the next terrain type, the switch estimator indicates when to switch to the next policy.}
% \caption{



% Our system uses a set of pre-trained policies and switch estimators, onefor each terrain condition. We run a single policy at a time, and switch when indicated by the switch estimator for the next policy. A policy is employed The current policy $i$ is employed, passing torques $a_i$ to the robot. When terrain condition $j$ is detected, we evaluate the output of switch estimator $e_j$, and switch the current policy to the next policy $j$ when indicated.

% We then switch to next policy $j$ when the switch estimator output $e_j$ indicates it is safe to switch.

% , and 
% As the next terrain condition $j$ is detected we evaluate the output of the switch estimator, $e_j$. 


% The robot state and heightmap are fed through the current policy
% $e$, $a$

% }

% \label{fig:method}
% \vspace{-3mm}
% \end{figure}


% The perception input is provided by a ground truth of box positions. If the centre of mass is over the current box, then we take current box $ + i$, where $i$ is from $[-1,0,1,2,3]$, i.e. we provide the information of the previous, current, and next 3 boxes relative to the robot centre of mass position. For each box, we provide two corners $x,y$ in robot frame, and $z$ relative to the height of the robot\brendan{should it be robot height? or z offset?}. In total there are $25$ numbers provided to the perception network \brendan{should these be normalised?}. Our perception decision enforces a limit on how close a the robot needs to be to an artifact to detect it.


% \brendan{Network information..
% The heightmap is fed into a convolutional neural network with two layers, and then is concatenated with the robot state, before being fed through two fully connected layers of size 128 before reaching the final layer. All subpolicies and estimators have the same network size.
% }

% We train a set of policies $\pi_i(s_t) \in \Pi$, including a base walking policy, and three terrain artifact policies. The terrain artifacts include stairs, a large gap, and a ledge that requires both feet of the robot to leave the ground.

% Each policy is trained with the same reward, changing the terrain in the second phase of the curriculum makes a policy specialise for a terrain type. Each terrain can walk on flat ground, though through terrain adaption each evolves a slight variant that differs from the original expert policy.


% learn a neural network approximator for $\mathcal{R}(\pi_i)(s_t)$ that predicts 

% by collecting data at transition states, and training an estimator to predict the likelihood of reaching a state in the goal se



% Sequential composition is the idea that moving from one state to another may involve executing several controllers in sequence~\cite{burridge_sequential_1999}. Conceptually, each controller has a set of states that form a funnel, where a robot in any state in the funnel will flow to a convex set of states known as the goal set. Each controller $\pi_i$ has a goal set
% $\mathcal{G}(\pi_i) = \{s_i^*\}$ and a Region of Attraction (RoA) $\mathcal{R}(\pi_i) = \{s_0 \in \mathcal{S} : \lim_{t\to\infty} s(t,s_0) = \mathcal{G}(\pi_i)\}$. $\mathcal{G}(\pi_i)$ is a set of states controller $\pi_i$ was designed to operate within, and $\mathcal{R}(\pi_i)$ is a set of states that will converge to a state in $\mathcal{G}(\pi_i)$. Thus $\mathcal{R}(\pi_i)$ acts as a funnel, moving any state $s_0$ in its set towards a state in $\mathcal{G}(\pi_i)$. Provided there exists an initial state $s_0\in \mathcal{R}(\pi_i)$, a common state in $\mathcal{G}(\pi_i)$ and $\mathcal{R}(\pi_j)$, and a target state $s_T \in \mathcal{G}(\pi_j)$, then $\pi_i$ can prepare $\pi_j$, shown in notation as $\pi_i \succeq \pi_j$, and therefore controllers can be backchained to move a robot through the state from $s_0$ to $s_T$. We consider switching between policies as a sequential composition problem, where terrain condition $j$ follows terrain condition $i$. \brendan{TODO, reduce this section/make it more relevant}


% how we can estimate when the currently executing policy $\pi_j$ has a RoA overlap between the next required policy $\pi_i$. 



% This switch e sw input 

% We consider the robot state and perception to be the same as for the policies.

% The complete set of states that make up the RoA for a walking controller is difficult to determine. Instead we estimate when the robot is in the RoA of the next policy by collecting data at transition states, and training an estimator to predict the likelihood of reaching a state in the goal set.

% Each policy $\pi_i$ has a goal set $\mathcal{G}(\pi_i)$. For a periodic controller, such as for walking, the goal set is all states visited by the unperturbed policy. For specific terrain artifacts, we define the goal set to be any state a suitable distance after the artifact where the robot maintains a CoM velocity and height typical during walking. 

% A key component to our method is that each element $\{\pi_i, \mathcal{G}(\pi_i),\mathcal{R}(\pi_i)\}$ is only obtained by interaction with terrain condition $i$. To better represent the distribution of transition states each policy may encounter, we first run controller $\pi_j$, where $j \neq i$, before switching to $\pi_i$. 

% Data is collected by running controller $j$ on terrain condition $i$ and switching to controller $i$ at a random distance after the terrain condition has been detected (Fig.~\ref{fig:estimator}a). Terrain detection occurs when the terrain artifact appears $0.9$m from the robot body, a distance consistent with the perception limit. Switching occurs at a distance sampled from $\mathcal{U}(0,0.9)$m from the artifact. We assume we have a method to detect the upcoming terrain type: the agent knows what controller it should use, we tell it when to switch.

% We collect a total of 5 data points when the controller is switched and assign each the same label, including the switch point and the surrounding two data points: $[t-2, t-1, t, t+1, t+2]$. This allows us to collect more data for each trial.

% A neural network is trained to minimise a mean squared error loss to estimate if the current robot state will likely reach the goal set for a given policy. The final layer of the network is a single output with a sigmoid activation. Data is split into 90\% training and 10\% validation, with a 50/50 split of positive and negative labels during training, and for validation. 





% \begin{figure}[tb!]
% \centering
% \subfloat[]{%
% \includegraphics[width=0.5\columnwidth]{images/plot_alive.png}}
% \hfill
% \subfloat[]{%
% \includegraphics[width=0.5\columnwidth]{images/plot_distance.png}}\hfill
% \hfill
% \subfloat[]{%
% \includegraphics[width=0.5\columnwidth]{images/plot_success.png}}\hfill
% \caption{a) Sim to real test platform, a torque controlled hexapod leg. b) Visualising the reality gap.}
% \label{fig:approach}
% \vspace{-3mm}
% \end{figure}

% \subsubsection{Success Prediction}



==> sections/method_old.tex <==
% \begin{figure}[tb!]
% \centering
% \includegraphics[width=1.0\columnwidth]{images/pic.png}
% \caption{We first train a set of subpolicies using a sequence of curricula (a-c) that ensures policies have a common set of states they work within as well increasing the stable region of each policy. We then learn where this overlap occurs by estimating the probability of success for switching between controllers in the current configuration $s_t$. Success is determined if the robot reaches a state in the goal set for the current controller ($\mathcal{G}(\pi_i)$). Finally we evaluate our method on an unseen test world of random artifacts.}
% \label{fig:method}    
% \vspace{-3mm}
% \end{figure}

\begin{figure}[tb!]
\centering
\includegraphics[width=1.0\columnwidth]{images/fig2.png}
\caption{
We pre-train a suite of deep reinforcement learning (DRL) policies for a set of terrain conditions, and each policy has a switch estimator. Using the current policy $i$, and detecting upcoming terrain type $j$, we use the switch estimator output $e_j$ to determine when the robot is in a suitable configuration to safely switch to the next policy $j$. Each policy $\pi_i$ (where $i \in$ $\{$walk, jump, gaps, stairs$\}$) is a neural network with inputs $s_t=\{$robot state, heightmap$\}$ and outputs $a_t$ that are the torques applied to each joint. Each switch estimator is a neural network with inputs $s_t=\{$robot state, heightmap$\}$ and outputs $e_j$, where $e_j \in [0,1)$ indicates that the current state is in the region of attraction (RoA) for policy $j$: $s_t \in R(\pi_j)$. Switching to $\pi_j$ is safest when $e_j$ is high.
}

\label{fig:method}
\vspace{-3mm}
\end{figure}

A summary of our method is outlined in Fig.~\ref{fig:method}. For each terrain type $i$, where $i \in$ $\{$walk, jump, gaps, stairs$\}$, we train a policy and a switch estimator. We use an oracle terrain detector to determine the upcoming terrain type, and therefore what the next policy will be. The switch estimator for the next policy is activated when the next terrain type is detected, with output $e_j$ indicating when the robot is in the RoA of the next policy: $s_t = \{$ robot state, heightmap $\} \in \mathcal{R}(\pi_j)$. We evaluate our method on a combination of terrain types and compare our method to several other methods for switching, as well as DRL methods that have been trained on the combination terrain set. 


\subsection{Problem definition}

% problem definition (where we talk about terrain types, what we are solving for, the robot state space, that we are given policies for each terrain type, assumptions like automatic detection of next terrain type, the input and output to the Switching Network. Specific terrain parameters (min, max height etc) should be parametrized and revealed in the Experiments section) 

% Plan is to move the state and perception stuff into the policy section. Does this make sense? The switching stuff relies on the robot state and hm, probably best to introduce before this section? Summary/Fig 2 -> Switching (plus sequential composition) -> Robot info (state, perception) -> Deep RL (MDP, PPO) -> sequential curriculum learning

The problem we consider is a biped in a 3D environment, with 12 torque controlled actuators using the Pybullet simulator~\cite{coumans_pybullet_nodate}. The task of the biped is to mimic a human last mile delivery driver, as such the robot must traverse stairs, gaps, and a large step. We are given a terrain detector that indicates the upcoming terrain.

The robot state consists of  $[J_t, Jv_t, c_t, c_{t-1}, CoM_t]$ where $J_t$ is the joint positions in radians, $Jv_t$ is the joint velocity in rad/s, $c_t$ and $c_{t-1}$ is the current and previous contact information of each foot (4 contact points per foot) and a flag for each foot indicating whether it should be in swing or stance, and $CoM_t$ is the linear and angular centre of mass velocities as well as pitch and roll positions and height above the terrain. In total there are $51$ elements to the robot state, which is normalised by subtracting the mean and dividing by the standard deviation.

Perception is provided in the form of a heightmap that moves with the x,y,z and yaw positions of the robot body, similar to work with simulated biped by~\cite{peng_deeploco_2017}. A heightmap is a common perception method used in robotics, usually extracted from range measuring sensors such as depth sensors, laser range sensors or stereo vision~\cite{koubaa_universal_2016}. Other work in DRL for walking uses perception from state information~\cite{lee_composing_2019}, RGB cameras~\cite{merel_hierarchical_2019}, or a heightmap~\cite{peng_deeploco_2017}. In early experiments, we found that using a heightmap improved policy performance compared with providing the ground truth terrain pose. The robot itself does not appear in the heightmap. The heightmap is clipped to be a maximum of 2m below the height of the robot, then scaled to be between 0 and 1. The heightmap has a resolution of $[60,40]$, with a grid size of $0.025$m. The robot is centred with a larger view in front. Its effective field of view is $0.9$m in front, $0.6$m behind, and $0.5$m to each side. A depiction of the heightmap is shown in Fig.~\ref{fig:method}. We consider the state $s_t$ to be the robot state and heightmap at time $t$.


\subsection{Learning When to Switch}

Switching from one policy to another by estimating when a state is in the RoA for the next policy is an idea that stems from the sequential composition framework~\cite{burridge_sequential_1999}. Each policy $\pi_i$ has a goal set $\mathcal{G}(\pi_i) = \{s_i^*\}$ and a Region of Attraction (RoA) $\mathcal{R}(\pi_i) = \{s_0 \in \mathcal{S} : \lim_{t\to\infty} s(t,s_0) = \mathcal{G}(\pi_i)\}$. $\mathcal{G}(\pi_i)$ is a set of states policy $\pi_i$ was designed to operate within, and $\mathcal{R}(\pi_i)$ is a set of states that will converge to a state in $\mathcal{G}(\pi_i)$. 

The complete set of states that make up the RoA for a biped traversing complex terrain types is difficult to determine. Instead we estimate when the robot is in the RoA of a policy by training a neural network switch estimator.

% . is the idea that moving from one state to another may involve executing several controllers in sequence
% Once we have trained each policy we no longer update their weights. Now we look at estimating when to switch between policies. We assume we are given an oracle terrain detector that indicates when a terrain artifact is in range of the robot perception system. This allows us to focus on switching (rather than also predicting the terrain type), otherwise our switching estimator would need data from every terrain type during training. Before we switch we need to know if the robot is in the RoA of the next policy. We train a switch estimator for each policy, predicting the probability of success for switching in the current state. 

Data is collected by running policy $j$ on terrain condition $i$ and switching to controller $i$ at a random distance from the terrain artifact (where $j \neq i$). As shown in Fig.~\ref{fig:estimator}a), there are three stages to data collection that occur for each sample: detection, switching, and labelling. Terrain detection occurs when the terrain artifact appears $0.9$m from the robot body. We switch to the target policy at a distance sampled from $\mathcal{U}(0,0.9)$m from the artifact. We label the sample as successful (1) if the robot reaches a goal zone (0.9m after the artifact), while maintaining a nominal CoM velocity and height. The sample is labelled as failed (0) otherwise.

We collect a total of 5 data points (robot state + heightmap) for each sample, including the data point when switching occurred at timestep $t$ and the surrounding two data points: $[t-2, t-1, t, t+1, t+2]$. This allows us to collect more data for each trial, while smoothing the switch estimator: states that are close should have a similar success prediction.

Each switch estimator $\mathcal{R}(\pi_i)$ is trained to minimise the loss $L(\phi) = (\mathcal{R}(\pi_i)(s_t) - y_t)^2$, where $\phi$ are the neural network weights, $s_t$ is the data point (robot state + heightmap), and $y_t$ is the label for data point $t$. The final layer of the network is a single output with a sigmoid activation. Data is split into 90\% training and 10\% validation, with a 50/50 split of positive and negative labels forced during training and validation. 

Each policy has its own switch estimator that is activated once its respective target terrain type is detected.  If we switch policies when the switch estimator for the upcoming policy predicts a high value, we increase the likelihood of the robot safely traversing the terrain.


\subsection{Training Policies}

% Learning when the robot is in the RoA of the next policy as a means of estimating when to switch can occur with any set of control policies, provided there exists a region of overlap between each expected policy switch. 

% We choose DRL as our method to populate our set of policies as it is difficult to design classical controllers to work over complex terrain~\cite{?}. 

% We could apply any method for obtaining policies, provided we are able to estimate when to switch
%  as it is difficult to design classical controllers to work over complex terrain~\cite{?}
Our switching method requires policies to have a RoA overlap, and provided this condition is met we could employ policies derived from any method. We choose DRL as our method to populate our set of policies. DRL approaches result in complex behaviours, though typically with policies that have a narrow RoA with little or no overlap between other policies. In this section we first introduce the reinforcement learning problem and algorithm of choice, we then introduce our reward function, and finally our curriculum learning approach that ensures policies have a RoA overlap. 

\subsubsection{Deep Reinforcement Learning}

We consider our task to be a Markov Decision Process (MDP) defined by tuple $\{\mathcal{S},\mathcal{A}, R, \mathcal{P}, \gamma\}$ where $s_t \in \mathcal{S}$, $a_t \in \mathcal{A}$, $r_t \in R$ are state, action and reward observed at time $t$, $\mathcal{P}$ is an unknown transition probability from $s_t$ to $s_{t+1}$ taking $a_t$, and $\gamma$ is a discount factor. 

% We use curriculum learning that uses external forces applied to the robot to guide initial learning. These forces are considered an artifact of the environment, therefore our MDP is evolving with the curriculum. For this reason we choose an on policy DRL algorithm, where we only keep a small replay history.

The reinforcement learning goal is to maximise the sum of future rewards $R = \sum_{t=0}^{T}\gamma^tr_t$, where $r_t$ is provided by the environment at time $t$. For continuous control, actions are sampled from a deep neural network policy $a_t\sim\pi(s_t)$, where $a_t$ is a torque applied to each joint.

We predict the value of being in each state $V(s_t) = r_t + \gamma V(s_{t+1})$, which is an estimate of the sum of future rewards $R$. We calculate an advantage from this prediction $A(s_t) = r_t + \gamma V(s_{t+1}) - V(s_t)$ that provides an estimate of how much better or worse action $a_t$ performed compared to what we expected. 

We update the policy $\pi(a_t|s_t)$ by scaling the log probability of taking action $a_t$ by the advantage $A(s_t)$ according to the loss function: $L(\theta) = \mathbb{E}[\log\pi_\theta(a|s)A(s)]$, where $\theta$ is the policy weights~\cite{schulman_proximal_2017}. Intuitively, if we did better than expected we want to increase the probability of performing that action next time, and if we did worse, reduce its probability.

In practice this loss can result in large updates to the policy that can adversely affect training. Instead we use a loss defined by Proximal Policy Optimisation (PPO)~\cite{schulman_proximal_2017}. PPO uses a surrogate loss that is clipped, ensuring policy predictions remain close to the predictions from the previous update. We also apply Generalised Advantage Estimation (GAE) as a low variance estimate of $A$~\cite{schulman_high-dimensional_2018}, leading to a more accurate prediction of $V(s_t)$ and faster convergence.  

% \subsection{Robot Information}

% Remove numbers (put in results).
\subsubsection{Reward Function}

Here we define the reward function used for each policy. In a previous work, motion capture is used to generated a target policy~\cite{peng_deepmimic_2018}. Instead of motion capture, we hand craft a target policy by designing a simple walking gait on a flat surface, without any simulator physics. Every terrain type uses the same target policy, even for the stair, jump, and gap terrains. We believe we could improve our policies and reduce training time if we designed a target policy for each terrain type, but for this work a common target policy worked sufficiently well for all polices. Our reward function is thus defined:
\[r_t = goal + pos + vel + CoM + step + act\]
where:
\begin{itemize}[leftmargin=*]
    \item $goal$ is the error between the body velocity and goal velocity $= w_{goal}\cdot \exp[c_{goal}\cdot e_{goal}]$.
    \item $pos$ is the error between the joint positions and the target joint positions $= w_{pos}\cdot \exp[c_{pos}\cdot e_{pos}]$.
    \item $vel$ is the error between the joint velocities and the target joint velocities (calculated with finite differences like~\cite{peng_deepmimic_2018}) $= w_{vel}\cdot \exp[c_{vel}\cdot e_{vel}]$.
    \item $CoM$ is the centre of mass error including deviations from a target height and zero roll and pitch positions $= w_{CoM}\cdot \exp[c_{CoM}\cdot e_{CoM}]$. 
    \item $step$ encourages stepping close to the middle of a step when in contact, as well as symmetrical step length ($left_x\approx right_x$ in contact) $= w_{step}\cdot \exp[c_{step}\cdot e_{step}]$. 
    \item $act$ is a penalty for excessive torque for each of the $n$ joints $= w_{act}\sum_n(a_t^2)$. 
\end{itemize}

Parameters $w$ and $c$ represent a tunable weighting for each element of the reward function, which is the same for each policy, and not changed during training. $e$ is the error of each respective element.

\subsubsection{Sequential Curriculum Learning}

Curriculum learning is a systematic way of increasing the difficulty of a task~\cite{bengio_curriculum_2009}, and results in learning an attractive walking gait quickly~\cite{yu_learning_2018}. We apply curriculum learning as a sequence of tasks: The first stage is learning to walk with target guidance on a flat surface, the second is a terrain curriculum where each policy is adapted to a specific terrain type, and the third stage introduces robustness to the polices by adding perturbations. 

% Policies must have a RoA overlap in order to switch. To ensure this happens we train each policy to have a common task during training: each policy starts from the same initial position, and must walk over flat terrain. We expand the RoA of each policy by adding external disturbances, increasing the robustness of each policy. To facilitate learning on complex terrain types with the aforementioned conditions, policies are trained using a sequence of curricula. The first stage is learning to walk with expert guidance on a flat surface, the second is a terrain curriculum where each policy is adapted to a specific terrain type, and the third stage introduces robustness to the polices by adding perturbations. 

The difficulty of each curriculum is increased as milestones are reached following work from~\cite{yu_learning_2018}. Unique to our method, we ensure each stage is completed before the commencement of the next stage, which we have found accelerates training. Average episode reward is used as the milestone for all stages: as the robot consistently achieves a threshold reward, the difficulty of the current curriculum is increased. 

To ensure RoA overlap, each policy must first stand for a random number of timesteps, then walk on a flat surface. We provide as additional input a velocity command input $v_t$. The velocity command parameter $v_t$ is concatenated with the robot state, which is set to 0 for standing, and 1 when the robot should move.  

\paragraph{First Stage - Learning to Walk}
The initial curriculum provides external forces to stabilise the centre of mass of the robot similar to~\cite{yu_learning_2018}. In addition, we provide an expert guided force at each actuator. Using our target walking policy introduced in the reward function section, we apply a target torque to each joint, calculated using a PD gain on the error between the robot joint positions and target joint positions. The target torque is added to the torque output from the policy. Importantly, the additional torque from the target PD controller is not considered in the gradient calculations of the policy, and is instead an artifact of the evolving environment. We found that providing this additional torque allows the robot to visit relevant parts of the state early in training, significantly increasing learning. The external forces, including the PD gain used to calculate the target torques, are annealed to zero before the next curriculum stage. Given each policy can walk on a flat surface after the first stage, an alternative approach could use a base walking policy as an initialisation for each policy. However, as the first stage is typically completed within the first 10\% of training, we simply train each policy from a random initialisation.

\paragraph{Second Stage - Adapting the Terrain}
After the first stage of training, each policy is capable of walking on a flat surface with no help from external forces. The terrain is slowly changed in the second stage, adding height to stairs and jumps, and length to gaps. Stairs are randomly selected as up or down. Gaps and jumps are added at random distance intervals with flat terrain otherwise. Each policy evolves to traverse its designated terrain condition, while sharing the same initial conditions. The second stage takes about 50\% of the training time (harder terrains take longer).

\paragraph{Third Stage - Adding External Perturbations}
In the final stage, and for the remainder of training, we add a curriculum of external perturbations. Adding random external forces is a way to improve the robustness of a policy~\cite{schulman_proximal_2017}, though too much noise early in training is a detrimental to learning. We apply an impulse force of random magnitude to the centre of mass in all 6 degrees of freedom of the torso. The force is sampled from a uniform distribution with a maximum value that is increased with each milestones. The force is applied for a single timestep (impulse), at random intervals of around 2 Hz. Having a dedicated curriculum for external disturbances allows us to use a large force that would otherwise prevent training if employed earlier. Once the third curriculum stage is complete, the maximum linear impulse force is 500N and the maximum torsional impulse force is 250Nm. In depth details and analysis of our sequential curriculum method is left for another work.




% \begin{figure}[tb!]
% \centering
% \includegraphics[width=1.0\columnwidth]{images/fig2.png}
% \caption{

% We pre-train a suite of policies for a set of terrain conditions, and each policy has a switch estimator. Using the current policy $i$, and detecting upcoming terrain type $j$, we use the switch estimator output $e_j$ to determine when the robot is in a suitable configuration to safely switch to the next policy $j$.

% We train a set of RL policies 
% $\pi_i$ on specific terrains where $i \in \{walk, jump, gaps, stairs\}$. 
% Each policy takes the state $s_t = \{robot state, heightmap\}$, and produces the next action, $a_t^i$ specifying the torques for each joint. Each policy also estimates $e_i \in [0,1)$ that the current state is in the region of attraction for this policy $s_t \in R(\pi_j)$. The upcoming policy $j$ is determined by a an assumed classifier of the terrain. The active policy $i$ is switched to $j$ when $e_j$ indicates the state, is in the region of attraction for the next policy .


% We train a set of RL policies $\pi_i$ on specific terrains where $i \in \{walk, jump, gaps, stairs\}$. Each policy takes the state S= {robot state, height map}, and produces the next action, $\a_i$ specifying the torques for each joint. Each policy also estimates $e_i \in [0,1)$ that the current state is in the region of attraction for this policy $S \ in R(\pi_j)$. The upcoming policy $j$ is determined by a an assumed classifier of the terrain. The active policy $i$ is switched to $j$ when $e_j$ indicates the state, is in the region of attraction for the next policy .

% We pre-train a suite of policies for a set of terrain conditions, and each policy has a switch estimator. Using the current policy $i$, and detecting upcoming terrain type $j$, we use the switch estimator output $e_j$ to determine when the robot is in a suitable configuration to safely switch to the next policy $j$.

% that determines when the robot is in a safe configuration for switching.

% For each policy $i$ we train a switch estimator with output $e_i$ that indicates when the robot is in a safe configuration to policy $i$.

% \caption{We train a set of policies $\pi$, and a switch estimator for each policy $\mathcal{R}(\pi)$. Each policy and switch estimator is trained on a single terrain artifact, we then evaluate our system in a test world with all artifact types. As the robot detects the next terrain type, the switch estimator indicates when to switch to the next policy.}
% \caption{



% Our system uses a set of pre-trained policies and switch estimators, onefor each terrain condition. We run a single policy at a time, and switch when indicated by the switch estimator for the next policy. A policy is employed The current policy $i$ is employed, passing torques $a_i$ to the robot. When terrain condition $j$ is detected, we evaluate the output of switch estimator $e_j$, and switch the current policy to the next policy $j$ when indicated.

% We then switch to next policy $j$ when the switch estimator output $e_j$ indicates it is safe to switch.

% , and 
% As the next terrain condition $j$ is detected we evaluate the output of the switch estimator, $e_j$. 


% The robot state and heightmap are fed through the current policy
% $e$, $a$

% }

% \label{fig:method}
% \vspace{-3mm}
% \end{figure}


% The perception input is provided by a ground truth of box positions. If the centre of mass is over the current box, then we take current box $ + i$, where $i$ is from $[-1,0,1,2,3]$, i.e. we provide the information of the previous, current, and next 3 boxes relative to the robot centre of mass position. For each box, we provide two corners $x,y$ in robot frame, and $z$ relative to the height of the robot\brendan{should it be robot height? or z offset?}. In total there are $25$ numbers provided to the perception network \brendan{should these be normalised?}. Our perception decision enforces a limit on how close a the robot needs to be to an artifact to detect it.


% \brendan{Network information..
% The heightmap is fed into a convolutional neural network with two layers, and then is concatenated with the robot state, before being fed through two fully connected layers of size 128 before reaching the final layer. All subpolicies and estimators have the same network size.
% }

% We train a set of policies $\pi_i(s_t) \in \Pi$, including a base walking policy, and three terrain artifact policies. The terrain artifacts include stairs, a large gap, and a ledge that requires both feet of the robot to leave the ground.

% Each policy is trained with the same reward, changing the terrain in the second phase of the curriculum makes a policy specialise for a terrain type. Each terrain can walk on flat ground, though through terrain adaption each evolves a slight variant that differs from the original expert policy.


% learn a neural network approximator for $\mathcal{R}(\pi_i)(s_t)$ that predicts 

% by collecting data at transition states, and training an estimator to predict the likelihood of reaching a state in the goal se



% Sequential composition is the idea that moving from one state to another may involve executing several controllers in sequence~\cite{burridge_sequential_1999}. Conceptually, each controller has a set of states that form a funnel, where a robot in any state in the funnel will flow to a convex set of states known as the goal set. Each controller $\pi_i$ has a goal set
% $\mathcal{G}(\pi_i) = \{s_i^*\}$ and a Region of Attraction (RoA) $\mathcal{R}(\pi_i) = \{s_0 \in \mathcal{S} : \lim_{t\to\infty} s(t,s_0) = \mathcal{G}(\pi_i)\}$. $\mathcal{G}(\pi_i)$ is a set of states controller $\pi_i$ was designed to operate within, and $\mathcal{R}(\pi_i)$ is a set of states that will converge to a state in $\mathcal{G}(\pi_i)$. Thus $\mathcal{R}(\pi_i)$ acts as a funnel, moving any state $s_0$ in its set towards a state in $\mathcal{G}(\pi_i)$. Provided there exists an initial state $s_0\in \mathcal{R}(\pi_i)$, a common state in $\mathcal{G}(\pi_i)$ and $\mathcal{R}(\pi_j)$, and a target state $s_T \in \mathcal{G}(\pi_j)$, then $\pi_i$ can prepare $\pi_j$, shown in notation as $\pi_i \succeq \pi_j$, and therefore controllers can be backchained to move a robot through the state from $s_0$ to $s_T$. We consider switching between policies as a sequential composition problem, where terrain condition $j$ follows terrain condition $i$. \brendan{TODO, reduce this section/make it more relevant}


% how we can estimate when the currently executing policy $\pi_j$ has a RoA overlap between the next required policy $\pi_i$. 



% This switch e sw input 

% We consider the robot state and perception to be the same as for the policies.

% The complete set of states that make up the RoA for a walking controller is difficult to determine. Instead we estimate when the robot is in the RoA of the next policy by collecting data at transition states, and training an estimator to predict the likelihood of reaching a state in the goal set.

% Each policy $\pi_i$ has a goal set $\mathcal{G}(\pi_i)$. For a periodic controller, such as for walking, the goal set is all states visited by the unperturbed policy. For specific terrain artifacts, we define the goal set to be any state a suitable distance after the artifact where the robot maintains a CoM velocity and height typical during walking. 

% A key component to our method is that each element $\{\pi_i, \mathcal{G}(\pi_i),\mathcal{R}(\pi_i)\}$ is only obtained by interaction with terrain condition $i$. To better represent the distribution of transition states each policy may encounter, we first run controller $\pi_j$, where $j \neq i$, before switching to $\pi_i$. 

% Data is collected by running controller $j$ on terrain condition $i$ and switching to controller $i$ at a random distance after the terrain condition has been detected (Fig.~\ref{fig:estimator}a). Terrain detection occurs when the terrain artifact appears $0.9$m from the robot body, a distance consistent with the perception limit. Switching occurs at a distance sampled from $\mathcal{U}(0,0.9)$m from the artifact. We assume we have a method to detect the upcoming terrain type: the agent knows what controller it should use, we tell it when to switch.

% We collect a total of 5 data points when the controller is switched and assign each the same label, including the switch point and the surrounding two data points: $[t-2, t-1, t, t+1, t+2]$. This allows us to collect more data for each trial.

% A neural network is trained to minimise a mean squared error loss to estimate if the current robot state will likely reach the goal set for a given policy. The final layer of the network is a single output with a sigmoid activation. Data is split into 90\% training and 10\% validation, with a 50/50 split of positive and negative labels during training, and for validation. 


\begin{figure}[tb!]
\centering
\subfloat[]{%
% \includegraphics[width=0.5\columnwidth]{images/estimator.png}}
\includegraphics[height=0.3\columnwidth]{images/estimator.png}}
\hfill
\subfloat[]{%
\includegraphics[height=0.3\columnwidth]{images/multi_roa.png}}
\hfill
\caption{a) A switch estimator is trained for each policy, with data collected from each terrain type separately. Data points (robot state and heightmap) are collected around the switch point and given a label of 1 if the robot reaches the goal state, 0 otherwise. b) Early switching is favourable for some policies, success is marked as green, whereas switching late is more likely to fail (red).}
\label{fig:estimator}
\vspace{-3mm}
\end{figure}


% \begin{figure}[tb!]
% \centering
% \subfloat[]{%
% \includegraphics[width=0.5\columnwidth]{images/plot_alive.png}}
% \hfill
% \subfloat[]{%
% \includegraphics[width=0.5\columnwidth]{images/plot_distance.png}}\hfill
% \hfill
% \subfloat[]{%
% \includegraphics[width=0.5\columnwidth]{images/plot_success.png}}\hfill
% \caption{a) Sim to real test platform, a torque controlled hexapod leg. b) Visualising the reality gap.}
% \label{fig:approach}
% \vspace{-3mm}
% \end{figure}

% \subsubsection{Success Prediction}



==> sections/related_work.tex <==

% \brendan{Classical control and needing primitives}
Controllers developed with bipedal robots with classical methods can perform complex behaviours such as ascending and descending stairs~\cite{ching-long_shih_ascending_1999}, balancing on a Segway~\cite{gong_feedback_2019}, and executing a jump~\cite{xiong_bipedal_2018}. Humanoid robots often employ a set of control primitives, each individually developed and tuned, such as Dynamic Movement Primitives which uses discrete and rhythmic controllers that allow a humanoid robot to play the drums and swing a tennis racket~\cite{schaal_dynamic_2006}. Hauser et al.~\cite{siciliano_using_2008} uses primitives to place and remove a foot from contact, enabling a robot to walk on uneven terrain, up a step, and climb a ladder. Motion capture primitives can be stitched together with Hidden Markov Models to create sequences of motions~\cite{kulic_incremental_2012}. Controllers developed with classical methods usually require extensive human engineering.

% \brendan{Classical Switching}
Linking a sequence of controllers together by understanding where each works has been demonstrated on a juggling robot, the stable switching of behaviours is known as sequential composition~\cite{burridge_sequential_1999}. A key component is determining the region of attraction (RoA) for each policy, which is defined as the set of states that whether engaging a given policy will converge to a target set of states defined for that policy. Estimating the RoA overlap between controllers can be difficult for robots with high state spaces, however it can be simplified by defining a set of pre and post conditions for each controller~\cite{faloutsos_composable_2001}, or by providing a rule-based bound on parameters like heading angle and switching frequency~\cite{gregg_control_2012}. 
Motahar et al~\cite{motahar_composing_2016} switch between straight, left turn, and right turn controllers operating a 3D simulated biped using reduced dimension hybrid zero dynamics control law. These methods result in combinations of complex primitives, though they require a mathematically defined RoA, or a hand designed switching criteria for each primitive. RoA expansion can also be considered to provide a greater overlap between controllers~\cite{borno_domain_2017}. Borno et al.~\cite{borno_domain_2017} estimates the RoA for a simulated humanoid using multiple forward dynamics model simulations, a similar approach to ours.

% \brendan{DRL}
DRL offers an alternative to classical control methods, policies learn how to act by interacting with the environment. DRL methods have demonstrated bipedal walking over complex terrain~\cite{schulman_proximal_2017,heess_emergence_2017,peng_deeploco_2017}, and performing complex maneuvers replicating motion capture~\cite{peng_deepmimic_2018}. Usually DRL methods are limited to solving a single task end-to-end, characterised by a scalar reward function. End-to-end methods require retraining if new terrains are introduced, and in a real setting it may be intractable to train on the complete set of expected conditions.

% \brendan{DRL with primitives}
Designing a single policy that can display multiple behaviours is challenging, and often results in the degraded performance of individual behaviours~\cite{lee_robust_2019}. Combining DRL primitives usually involves training a deep Q network (or a similar discrete switching network) that selects which primitive to use~\cite{liu_learning_2017,merel_hierarchical_2019,lee_robust_2019}, or learning a complex combination of primitives~\cite{peng_mcp_2019}. Other hierarchical approaches learn the primitives and selection network together~\cite{bacon_option-critic_2018}, or with several task-dependent selection networks~\cite{frans_meta_2017}. Training in each of these examples needs access to all expected environment conditions during training, and adding new primitives requires retraining of the selection policy.

% \brendan{DRL with RoA estimation    }
While estimating the complete RoA of a policy is possible for systems with a relatively small state space, such as the single~\cite{berkenkamp_safe_2017},~\cite{najafi_learning_2016}, or double inverted pendulum~\cite{randlov_combining_2000}, for more complex systems the RoA is difficult to determine. Where it is possible to differentiate between unmodeled regions of the state from those that are well behaved, DRL can guide the agent back to where a classical controller can take over~\cite{najafi_learning_2016},~\cite{randlov_combining_2000}. Other work with DRL has shown that expanding the RoA of each primitive with transition policies improves switching~\cite{lee_composing_2019}. Designing policies with DRL for complex walking robots and  combining these behaviours with RoA estimation is a promising approach to scale the capabilities of legged robots, and is an area of research that requires more investigation. 

% \brendan{Our work}
In our work, we pre-train a set of policies with DRL to traverse complex terrain artifacts. We not only ensure there is a RoA overlap between policies, but also estimate when the overlap occurs such that policies can be switched safely, without the need to train on the complete set of terrain combinations.
% Dynamic humanoid robots have a state space that is very large, with a RoA that is narrow. Expanding the RoA is an approach to ensure sequential policies have a RoA overlap, where switching can safely occur in these states,~\cite{lee_composing_2019}. 
% ~\cite{randla_combining_2000}

% DRL methods that use a switching policy to combine pre-trained policies require activating each policy on all expected terrain conditions during training,, which may be prohibitive in a real setting. Furthermore, any new policy added to the suite requires retraining of the switching mechanism.



% Region of Attraction in RL
% While estimating the complete RoA is possible for systems with a smaller state space~\cite{berkenkamp_safe_2017},~\cite{najafi_learning_2016}, for many systems the RoA is difficult to determine. Dynamic humanoid robots have a state space that is very large, with a RoA that is narrow. Expanding the RoA is an approach to ensure sequential policies have a RoA overlap, where switching can safely occur in these states~\cite{borno_domain_2017},~\cite{lee_composing_2019}. 


% A key advantage of DRL over classical methods is policies that learn to act directly from perception. Perception is advantageous for walking over complex terrain, whether from state information~\cite{lee_composing_2019}, RGB camera~\cite{merel_hierarchical_2019}, or a heightmap~\cite{peng_deeploco_2017}. Resulting policies can walk over narrow paths~\cite{peng_deeploco_2017}, over steps~\cite{heess_emergence_2017}, avoid obstacles, and plan with visual queues~\cite{merel_hierarchical_2019}.

==> sections/related_work_old.tex <==
\begin{itemize}
    \item a. Walking Robots in Classical Control
    \item b. Walking Robots in Deep RL
    \item c. Policy Switching
    \item Our method, short
\end{itemize}

It is difficult to make controllers for walking robots for complex terrain types. Maybe its good to make one policy per terrain type, then learn when to switch between policies.

\subsection{Classical Control of Walking Robots}

It is difficult to design policies using classical control methods. 
Examples of why it is hard to classically make a controller for a walking robot. Why do we need multiple policies.
- cassie on a segway
- Anymal multi policy paper~\cite{lee_robust_2019}


\subsection{Deep Reinforcement Learning for Walking Robots}
% Examples of how DRL can help with some of the problems with classical methods.
% Deep RL for complex terrain types
Deep reinforcement learning (DRL) methods have demonstrated impressive results for the control of walking robots in simulation~\cite{heess_emergence_2017},~\cite{schulman_proximal_2017},~\cite{xie_feedback_2018},~\cite{peng_deepmimic_2018} and on real systems~\cite{hwangbo_learning_2019},~\cite{peng_learning_2020},~\cite{haarnoja_soft_2019}. 

\subsection{Policy Switching}

There are many examples of using a suite of policies to extend the capabilities of walking robots~\cite{frans_meta_2017},~\cite{merel_hierarchical_2019},~\cite{lee_composing_2019},~\cite{peng_mcp_2019},~\cite{lee_robust_2019}. Other hierarchical DRL algorithms learn subpolicies concurrently with a policy selector ~\cite{bacon_option-critic_2016}, or through mixed level control~\cite{peng_deeploco_2017}. A common theme and central limitation for these methods is they learn through interaction with the test domain: during training the learning algorithm must see all terrain combinations. This may be difficult in real world setting. Also, as new controllers are required, retraining of the switch mechanism is also required.

Classical methods for switching between controllers employ sequential composition~\cite{burridge_sequential_1999}, the idea that a sequence of controllers can be chained together by understanding where each controller works in the state space. 

Sequential composition requires an overlap between states that controllers operate. For dynamic humanoid robots the state space is very large, and the region that a controller is stable is narrow.~\cite{borno_domain_2017} proposed a method to expand the RoA of controllers for a simulated humanoid by finding a trajectory between a query state and a state in the RoA. Knowing this stable region is difficult. In their work,~\cite{faloutsos_composable_2001} define a set of pre and post conditions for each candidate controller, such that a supervisor policy can determine when a controller may be employed, and when it has completed its behaviour.

When there is no overlap between controllers, DRL can be used to train a new controller to complete the chain.~\cite{najafi_learning_2016} train a swing up policy for an inverted pendulum to work with a hand designed control policy for keeping the pendulum upright. For systems where the RoA can be estimated,~\cite{berkenkamp_safe_2017} demonstrate safe exploration while training a DRL agent, also using an inverted pendulum.

% Methods for switching between policies






% Classical methods for switching between controllers employ sequential composition~\cite{burridge_sequential_1999}, the notion that a sequence of controllers can be chained together by understanding where each controller works in the state space. 

% Sequential composition requires an overlap between states that controllers operate. For dynamic humanoid robots the state space is very large, and the region that a controller is stable is narrow.~\cite{borno_domain_2017} proposed a method to expand the RoA of controllers for a simulated humanoid by finding a trajectory between a query state and a state in the RoA. Knowing this stable region is difficult. In their work,~\cite{faloutsos_composable_2001} define a set of pre and post conditions for each candidate controller, such that a supervisor policy can determine when a controller may be employed, and when it has completed its behaviour.

% When there is no overlap between controllers, DRL can be used to train a new controller to complete the chain.~\cite{najafi_learning_2016} train a swing up policy for an inverted pendulum to work with a hand designed control policy for keeping the pendulum upright. For systems where the RoA can be estimated,~\cite{berkenkamp_safe_2017} demonstrate safe exploration while training a DRL agent, also using an inverted pendulum.
 
% DRL policies require carefully designed reward functions. It is common for policies trained with naive reward signals to behave unrealistically~\cite{schulman_proximal_2017},~\cite{heess_emergence_2017}. For robots that have human or animal characteristics, reward signal can be adapted from motion capture data~\cite{peng_deepmimic_2018},~\cite{merel_hierarchical_2019}, resulting in policies that transfer effectively to real legged platforms~\cite{peng_learning_2020}. 

% A common drawback of DRL methods is inefficient training time, where policies take millions of iterations with the environment~\cite{schulman_proximal_2017}. Using curriculum learning this process can be expedited~\cite{yu_learning_2018}. Recent off-policy algorithms are sample efficient enough to train directly on real platforms~\cite{haarnoja_soft_2019}, though the latest work in simulation-to-real transfer shows successful real world transfer of policies trained only in simulation~\cite{hwangbo_learning_2019}, or through a handful of real world iterations~\cite{peng_learning_2020}.

≥% Perception is advantageous for walking over complex terrain, whether from state information~\cite{lee_composing_2019}, RGB camera~\cite{merel_hierarchical_2019}, or a heightmap~\cite{peng_deeploco_2017}. With DRL, visuomotor policies directly learn to act in response to a perception signal. This results in policies that can walk over narrow paths~\cite{peng_deeploco_2017}, over steps~\cite{heess_emergence_2017}, avoid obstacles, and plan with visual queues~\cite{merel_hierarchical_2019}.

% Our method shares properties of several of these works. We use expert guidance like~\cite{peng_deepmimic_2018} to train attractive walking policies, as well as curriculum learning adapted from~\cite{yu_learning_2018} to train on complex terrain types.

% We expand the RoA of each policy, while ensuring an overlap between policies. Unlike other methods that also use pre-trained policies~\cite{merel_hierarchical_2019},~\cite{lee_composing_2019}, our method does not require training on the test domain. Instead we train all components of our system separately on single terrain conditions, and validate our results on the test environment where our system experiences the full combination of terrain artifacts for the first time.

% If we know the states that will result in a stable configuration for the robot using a particular controller (the controllers RoA), then we can confidently switch while in this state to a controller move the robot through the state to target locations.

% ere a controller works, we can execute a sequence of controllers, only switching when we are in the RoA for the next controller.

% Each controller is designed to work in a set of states known as the goal set. Any state for which a specified controller will converge to its goal set is said to be in the region of attraction (RoA) for that controller

% A more general framework is found in the control literature as sequential composition~\cite{burridge_sequential_1999}. The central idea is that each controller works for a known set of states referred to as the goal set. Any state for which a specified controller will converge to its goal set is said to be in the region of attraction (RoA) for that controller.\footnote{Region of Attraction is also known as Domain of Attraction, we use Region of Attraction in this work} Each controller forms a funneling behaviour where a state that is in the RoA for a specified controller will move towards a state in its goal set. If the goal set for one controller is present in the RoA for another, controllers can be backchained such that a robot could move from an initial state in the RoA of one controller towards a target state that is in the goal set of another. ~\cite{burridge_sequential_1999} demonstrated sequential composition with a ball juggling robot. 



% To extend the capabilities of a legged system to a similar range as our human delivery driver, we need a complex system of controllers. While end-to-end methods may be possible in simulation~\cite{peng_deeploco_2017},~\cite{heess_emergence_2017},~\cite{schulman_proximal_2017},~\cite{xie_feedback_2018},~\cite{peng_deepmimic_2018}, it is far more difficult to train a single policy for all terrain types on a real system. 





% Deep reinforcement learning (DRL) methods have demonstrated impressive results for the control of walking robots in simulation~\cite{peng_deeploco_2017},~\cite{heess_emergence_2017},~\cite{schulman_proximal_2017},~\cite{xie_feedback_2018},~\cite{peng_deepmimic_2018}. 

% \nick{you need to split up DRL into end to end, and the set of policies - like the heireacharle paper}

% There are several key advantages of DRL policies over traditional control design that make them suitable for walking robots.\footnote{We use the terms policy and controller interchangeably.} A key benefit is not having to model the dynamics of the system, instead a policy is trained through interaction with the environment. For highly dynamic bipedal motion, DRL method result in policies capable of complex maneuvers, such as jumping and flips, with very little manual control design~\cite{peng_deepmimic_2018}. 

% \nick{I object to you saying you don't model the dynamics- you are using a simulator model of the dynamics. I think the key benefit is that you don't need years of engineering! - but the best walking algorithms are still seemingly made by hand on real robots}

% Perception is advantageous for walking over complex terrain. With DRL visuomotor policies directly learn to act in response to a provided perception signal. This results in policies that can walk over narrow paths~\cite{peng_deeploco_2017}, over steps~\cite{heess_emergence_2017}, avoid obstacles, and plan with visual queues~\cite{merel_hierarchical_2019}. 

% DRL policies require carefully designed reward functions. It is common for policies trained with naive reward signals to behave unrealistically~\cite{schulman_proximal_2017},~\cite{heess_emergence_2017}. For robots that have human or animal characteristics, reward signal can come from motion capture data~\cite{peng_deepmimic_2018},~\cite{merel_hierarchical_2019}, resulting in realistic policies that transfer effectively to real legged platforms~\cite{peng_learning_2020}. 

% A common drawback of DRL methods is inefficient training time, where policies take millions of iterations with the environment. Using curriculum learning this process can be expedited, and more realistic policies encouraged~\cite{yu_learning_2018}. Recent off-policy algorithms are sample efficient enough to train directly on real platforms~\cite{haarnoja_soft_2019}, though the latest work in sim2real transfer shows successful real world transfer of policies trained only in simulation~\cite{hwangbo_learning_2019}, or through a handful of real world iterations~\cite{peng_learning_2020}.

% To extend the capabilities of legged systems to a similar range as our human delivery driver, we need a more complex system of controllers. While end-to-end methods may be possible in a simulation, it is far more difficult to train a single policy for all terrain types on a real system. Traditional hierarchical reinforcement learning methods also suffer with training on the test set, where low and high level controllers are trained concurrently~\cite{peng_deeploco_2017}, or in a temporally extracted hierarchy as in the options framework ~\cite{bacon_option-critic_2016}, both requiring interaction with the test domain. Other examples that utilise pre-trained policies train a selector policy that learns when to employ each primitive~\cite{merel_hierarchical_2019},~\cite{lee_composing_2019}. In each of these cases the robot would need to have access to the complete selection of terrain conditions while training, a condition that may be difficult for a real system.

% Alternatively, defining separate controllers as necessary means the capabilities of the robot can grow in a modular way. The work of~\cite{faloutsos_composable_2001} defines a set of pre and post conditions for each candidate controller, such that a supervisor can determine when a controller may be employed, and when it has completed its behaviour. 

% A more general framework is found in the control literature as sequential composition~\cite{burridge_sequential_1999}. The central idea is that each controller works for a known set of states referred to as the goal set. Any state for which a specified controller will converge to its goal set is said to be in the region of attraction (RoA) for that controller.\footnote{Region of Attraction is also known as Domain of Attraction, we use Region of Attraction in this work} Each controller forms a funneling behaviour where a state that is in the RoA for a specified controller will move towards a state in its goal set. If the goal set for one controller is present in the RoA for another, controllers can be backchained such that a robot could move from an initial state in the RoA of one controller towards a target state that is in the goal set of another. ~\cite{burridge_sequential_1999} demonstrated sequential composition with a ball juggling robot. 

% Sequential composition requires an overlap between controllers. For dynamic humanoid robots the state space is very large, and the region that a controller is stable is narrow.~\cite{borno_domain_2017} proposed a method to expand the RoA of controllers for a simulated humanoid. 

% When there is no overlap between controllers, DRL can be used to train a new controller to complete the chain. Using DRL, ~\cite{najafi_learning_2016} train a swing up controller for an inverted pendulum to work with analytical controllers.~\cite{lee_composing_2019} learn transition policies for each control primitive that act to expand the RoA of the subsequent controller.

% % Hierarchy of RoA: non-holonomic paper

% Our method shares properties of several of these works where we use curriculum learning to train attractive walking policies similar to~\cite{yu_learning_2018} and~\cite{peng_deepmimic_2018}, and train a success prediction function similar to the proximity predictor used by~\cite{lee_composing_2019} to estimate when to switch between policies. Unlike~\cite{lee_composing_2019}, our estimator is trained only on a single artifact type, with the combination terrain withheld for validation.

% As shown by~\cite{berkenkamp_safe_2017}, safe learning in the region of attraction..

% Lyapanouv neural network ~\cite{richards_lyapunov_2018}


% For more complex simulated agents, transition policies provide the RoA overlap. 


% While it is difficult to compute the RoA for complex robot, 


% Other papers from doc

% Anymal paper

% simulated humanoid robot must
% Each controller must come with means for identifying when it should be employed, and a way to switch from the current controller. For a complete system, there should always 



% Legged robots that  that they can traverse unstruct, where it is un

% As we scale the capability of robots, we scale where they need to operate. Legged systems that are able to traverse a range of terrain types require a set of controllers.  , autonomously selecting controllers based on terrain types

% Sequential composition and Learning policy primitives




% Complex walking tasks require several policies to be used sequentially. 
% Composing controllers 

% Merel primitives


% Restate the problem: walking controllers are hard, DRL makes things easier, (DRL examples), to increase the capabilities of our robot we might need lots of controllers, combining policies are necessary, we have learned when to switch policies to improve success.


% The limitations of DRL 
% Limitations - reward design, time, sim2real

% is visuomotor policies. through incorporating perception information directly into the control policy in what is known as visuomotor policies, where a controller can learn to respond to terrain changes without expl 

% DRL derived control policies are usually designed for a specific task, characterised by a training domain and a crafted reward function. 

% As the capabilities of these controllers extend to more complex terrain types, we , so does the need to glue together policies such that a robot can traverse a wide scope of terrain types. For highly a dynamic robot such as a biped, control policies work in a very narrow set of joint configurations and state conditions such that deviation from these conditions results in instability. The difficulty then comes in estimating when to switch between given policies such that success with the 

% Using control primitives to 

% Region of attraction


% Sequential composition refers to a paper~\cite{burridge_sequential_1999}

% Composing controllers paper~\cite{faloutsos_composable_2001}




% expanding roa paper

% Deep reinforcement learning has for walking robots~\cite{hwangbo_learning_2019}, cassie one.


==> sections/results.tex <==
% \subsection{Subpolicies}

% Training curves? Should have some way of testing the claim that policies have overlapping RoA's.

% \subsection{Region of Attraction Estimation}

% \brendan{Should I do the same comparisons on the single environments?}

% We show the baseline results of running each subpolicy on their respective terrain artifacts in Fig.~\ref{tab:roa_results}.
% training on each individual artifact, comparing baselineOur switching method is compared to several other methods, with results displayed in Table.~\ref{tab:roa_results}.


% \begin{table}[]
%     \centering
%     \begin{tabular}{c|c|c|c}
%          & Baseline & Switch Estimate\\   
%          \hline
%          Jumps  & 0.53 &  0.63\\
%          Gaps  & 0.53 &  0.63\\
%          Stairs  & 0.53 &  0.63\\
%          Base  & 0.53 &  0.63\\
%          Zero  & 0.53 &  0.63
%     \end{tabular}
%     \caption{Caption}
%     \label{tab:roa_results}
% \end{table}

% stairs: Thres 0.00 time alive: 0.7091 distance travelled: 0.6733  success: 0.3440
% jumps: Thres 0.00 time alive: 0.9804 distance travelled: 0.9398  success: 0.9120
% gaps: Thres 0.00 time alive: 0.8088 distance travelled: 0.7876  success: 0.6040
% Thres 0.00 time alive: 0.9974 distance travelled: 0.8012  success: 0.8140

% \subsection{Subpolicies}

% \noindent
% \begin{minipage}{0.75\linewidth}

% First version: Many vertical lines, 
% widths of horizontal lines all equal, 
% spacing above\slash below horizontal 
% lines cramped

% \smallskip
% \begin{minipage}{0.9\linewidth}
% \begin{tabularx}{\textwidth}{ |c| *{6}{Y|} }
% % \begin{tabularx}{\textwidth}{ |c| *{6}*{columnwidth/6|} }
% % \begin{tabularx}{\textwidth}{ |c| *{6}*{0.5|} }
% \cline{2-7}
%   \multicolumn{1}{c|}{} 
%  & \multicolumn{3}{c|}{Fantastical aardvarks}  
%  & \multicolumn{3}{c|}{Spelunking elephants}\\
% \hline
%  Foo bar & A & B & C & A & B & C\\
% \hline
%  5  & 87 &  5 &  2 & 82 & 18 & 48\\
%  6  &  5 & 43 &  4 &  7 & 47 &  4\\
%  7  &  7 & 18 & 63 &  2 &  9 & 99\\
% \hline
% \end{tabularx}
% \end{minipage}

% ****** EXAMPLE TABLE ***************
% \begin{minipage}{0.95\linewidth}
% \begin{tabularx}{\textwidth}{c *{6}{Y}}
% \toprule
% Foo bar
%  & \multicolumn{3}{c}{Fantastical aardvarks}  
%  & \multicolumn{3}{c}{Spelunking elephants}\\
% \cmidrule(lr){2-4} \cmidrule(l){5-7}
%   & A & B & C & A & B & C\\
% \midrule
%  5  & 87 &  5 &  2 & 82 & 18 & 48\\
%  6  &  5 & 43 &  4 &  7 & 47 &  4\\
%  7  &  7 & 18 & 63 &  2 &  9 & 99\\
% \bottomrule
% \end{tabularx}
% \captionof{table}{\textbf{How is Regional Accounting Information Processed by Real Estate Forecasters?}}
% \label{tab:1}
% \end{minipage}
% ****** EXAMPLE TABLE ***************

% \begin{minipage}{0.95\linewidth}
% \begin{tabularx}{\textwidth}{c *{7}{Y}}
% \toprule
% %  \multicolumn{7}{c}{Parameter Weights of the Reward Function}\\  
% %  \midrule
% %  & \multicolumn{3}{c}{Spelunking elephants}\\
% % \cmidrule(lr){2-4} \cmidrule(l){5-7}
%   & Goal   & Pos & Vel & CoM & Step & Act \\
% \midrule
%   $w$  & 1.0 & 0.65 & 0.05 & 0.1 & 0.2 & - \\        
%   $c$   & -3.0 & -2.0 & 0.1 & -10.0 & -5.0 & -0.0001 \\
% \bottomrule
% \end{tabularx}
% \captionof{table}{Weights used in the reward function.}
% \label{tab:params}
% \end{minipage}

% Parameters
% \begin{table}[]
%     \centering
%     % \begin{tabular}{c|c|c|c|c|c|c}
%     \begin{tabular}{x{0.9cm}|x{0.9cm}|x{0.9cm}|x{0.9cm}|x{0.9cm}|x{0.9cm}|x{0.9cm}}
%     % \begin{tabular}{p{2cm}|p{2cm}|p{2cm}}
%          \hline
%   & Goal   & Pos & Vel & CoM & Step & Act \\
%          \hline
%   $w$  & 1.0 & 0.65 & 0.05 & 0.1 & 0.2 & - \\        
%   $c$   & -3.0 & -2.0 & 0.1 & -10.0 & -5.0 & -0.0001 \\
%          \hline
%     \end{tabular}
%     \caption{Parameters used in the reward function.}
%     \label{tab:params}
% \end{table}



% \brendan{I'm not sure where this goes:}

% The parameters used in the reward function are given in Table~\ref{tab:params}. 
In this section, we present the results of our simulation experiments. First, in Sec~\ref{sec:single} we analyze the performance of each policy on the single artifact type they are trained on. Second, in Sec~\ref{sec:multi} we present results on terrains that have a sequence of randomly ordered multiple artifact types. In Sec~\ref{sec:comparison} we discuss how our approach compares with learning methods that are trained directly on the multi-terrains. For performance evaluation, we measure two metrics: 
\begin{itemize}
\setlength\itemsep{0pt}
    \item \textbf{\% Total Distance:} How far the robot has travelled as a percentage of the total terrain length.
    \item \textbf{\% Success:} The percentage of cases where the robot was able to get to the end of the terrain without falling.
\end{itemize}

Each terrain artifact is made up of horizontally stacked boxes, with each trial composed of 7 artifacts. In the single-terrain case all artifacts are of the same type, whereas in the multi-terrain case they are randomly selected among all terrain types. Terrain artifacts consist of Stairs (up and down) with a rise of 0.17m, Gaps that are 0.7m in length, and Steps 0.3m high and 0.16m in length. The terrain width is sampled uniformly from $\mathcal{U}(1.1,1.7)$m and fixed for each trial, flat segments (including the run of stairs) have a length sampled uniformly from $\mathcal{U}(0.36,0.44)$m. We do not consider the efficacy of policies on terrains outside of these ranges, some discussion on out of distribution operation is presented in~\cite{tidd_guided_2020}. 

% Each terrain artifact is made up of horizontally stacked boxes, with each trial composed of exactly 7 artifacts. In the single-terrain case all artifacts are of the same type, whereas in the multi-terrain case they are randomly selected among all terrain types. Each box has a width sampled from $\sim\mathcal{U}(1.1,1.7)$m. Flat segments have a length sampled from $\sim\mathcal{U}(0.36,0.44)$m. Terrain artifacts consist of stairs (up and down) with a rise of 0.17m, gaps of 0.7m in length, and steps that are 0.3m. Gaps and steps have a fixed length of 0.7 and 0.16m respectively. 

%  Each box length (except for the gaps and jumps artifact) are sampled from $\mathcal{U}(0.36,0.44)$, this is different from artifact training where box lengths are fixed for a whole trial.
\subsection{Single Artifact Type Terrains}
\label{sec:single}

Table~\ref{tab:individual_results} shows the percentage of total track distance covered and the success rate for each terrain type. Each policy is evaluated for 500 trials with 7 artifacts per trial. In these results no switching occurs. The Walk policy had the highest success rate with 99.2\%, which was expected because the robot was on flat surface. Jumps policy on step artifacts performed second best, with 91.2\% success rate. The Gaps and Stairs policies were the least successful, reaching to the final zone only 60.4\% and 34.4\% of the time. Percentage of the total distance metric was consistent with the success rates.

% \brendan{Statement about these results? What do they mean, why is the success rate so low for stairs (and gaps)? Should it correlate/provide an upper bound to switching?}
% Thres 0.00 time alive: 0.9955 distance travelled: 0.9766  success: 0.9920
% \smallskip
% \begin{minipage}{0.7\linewidth}
% \begin{tabularx}{\textwidth}{c| *{3}{Y}}
% \toprule
% \multicolumn{3}{c}{Results of 500 Trials on a Single Terrain World}\\
% \midrule
%  Artifact Type & Percentage of Total Distance & Success Rate \\   
% \midrule
%          Walk   & 0.9766 & 0.9920 \\
%          Jumps  & 0.9398 & 0.9120 \\
%          Gaps   & 0.7876 & 0.6040 \\
%          Stairs & 0.6733 & 0.3440 \\
% \bottomrule
% \end{tabularx}
% \captionof{table}{Weights used in the reward function.}
% \label{tab:individual_results}
% \end{minipage}

% |p{3cm}||p{3cm}|p{3cm}|p{3cm}| 
\begin{table}[]
    \vspace{3mm}
    \centering
    % \begin{tabular}{c|c|c|c|c|c|c|c}
    % \begin{tabular}{c|c|c}
    % \begin{tabular}{|c|cc|cc|}

    % \begin{tabular}{p{1.cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}}
    \begin{tabular}{p{1.cm}|M{1.75cm}|M{1.5cm}|M{1.75cm}|M{1.5cm}}
    % \begin{tabular}{p{2cm}|p{2cm}|p{2cm}}
         %\hline
         %\multicolumn{3}{c}{Results of 500 Trials on a Single Terrain World}\\
        %  \hline
        % %  Policy & \% Total Dist. & \% Success \\   
        %  Policy & \multicolumn{2}{c|}{\% Total Dist.} & \multicolumn{2}{c|}{\% Success}\\
        %  \hline
        % %  Walk   & \textbf{97.6} & \textbf{99.2} \\
        %  Walk   & \multicolumn{2}{c|}{\textbf{97.6}} & \multicolumn{2}{c|}{\textbf{99.2}} \\
        %  Jumps  & 93.9 & 86.2 & 91.2 & 77.5\\
        %  Gaps   & 78.7 & 87.4 & 60.4 & 75.5 \\
        %  Stairs & 67.3 & 78.7 & 34.4 & 59 \\
         
         Policy & \% Total Dist. &\% Success & \% Total Dist. no Overlap & \% Success  no Overlap\\
         \hline
        %  Walk   & \textbf{97.6} & \textbf{99.2} \\
        %  Walk   & \textbf{97.6} & \textbf{99.2} & \textbf{97.6} & \textbf{99.2}\\
         Jumps  & 93.9 & 91.2 & 86.2 & 77.5\\
         Gaps   & 78.7 & 60.4  & 87.4 & 75.5 \\
         Stairs & 67.3 & 34.4  & 78.7 & 59 \\
         
        
        % Original format and results:
        % \hline
        % Policy & \% Total Dist. & \% Success \\ 
        % \hline
        %  Walk   & \textbf{97.6} & \textbf{99.2} \\
        %  Jumps  & 93.9 & 91.2 \\
        %  Gaps   & 78.7 & 60.4 \\
        %  Stairs & 67.3 & 34.4 \\
         
         \hline
    \end{tabular}
    \caption{Results of each individual policy on its corresponding terrain type (i.e. Walking policy on flat terrain). \% of total track distance covered and \% success is shown. We also report the success of policies that are trained without explicit RoA overlap.}
    \label{tab:individual_results}
\end{table}

% \subsection{Test World}

\subsection{Multiple Artifact Type Terrains}
\label{sec:multi}
Our switching method is compared with several other methods, with results displayed in Table~\ref{tab:test_results}. All tests are performed with 2500 trials of a test world consisting of 7 terrain artifacts randomly selected from gaps, jumps and stairs. Each trial begins with a flat segment and the walk policy. Artifacts are restricted so there may not be two sequential artifacts of the same type. For the combination test worlds, only widths are fixed for an episode, each box length is randomly chosen. The number of boxes in each artifact varies from 4 to 9, while ensuring at least 0.9m of flat surface before each artifact to be consistent with how our switch estimator data is collected.

% While training policies, the terrain for an episode has a fixed length and width. 



%\subsubsection{Comparisons}

We compare our policy switching method with several heuristic methods, with the only difference between the methods being the timing of the switching.
\begin{itemize}[leftmargin=*]
    \item \textbf{Random:} Switching occurs a random distance after the artifact is detected.
    \item \textbf{On detection:} Switching occurs as soon as a next artifact is detected.
    \item \textbf{Lookup table:} We evaluate the optimal distance to switch for all switch combinations. On each artifact separately, we record the success rate of switching from any other policy to the target policy from 0 to 0.9m from the artifact (0.01m resolution).  Therefore, each switchable combination (e.g. $\pi_j$ to $\pi_i$) has a table of size $90$. We then take the $\arg\max$ of each permutation to determine the optimal switch distance for each artifact given the current policy and the target policy.
    \item \textbf{Centre of mass over feet:} Having the CoM over the support polygon created by the grounded foot is a well known  criteria for the stability of legged robots~\cite{faloutsos_composable_2001}. We switch when the following two conditions are true: 1) CoM is over the support polygon and 2) Both feet are within a tolerance distance to each other.%, switching when these conditions are met encourages RoA overlap as all policies share this configuration.% If the condition is not met and the robot is within 1cm of the artifact, switching is forced.
    \item \textbf{Our switch estimator:} We predict the probability of success for switching in the current state with our switch estimators. We threshold our predictions at 0.85 which empirically gave the best overall success for transitions. If terrain condition $i$ is detected and $\mathcal{E}_i(s_t) \geqslant 0.85$ we switch to $\pi_i$. 
    \item \textbf{Our switch estimator without region of attraction overlap:} We test our method using policies trained without considering a region of attraction overlap. The robot is initialised from a random set of joint positions, and is not required to pause before commencing locomotion. All other training and terrain properties are  consistent with our switch estimator method, and all policies achieve comparable, or better success rates to those reported in Table.~\ref{tab:individual_results}.
\end{itemize}

For \textbf{CoM over feet} and our \textbf{Switch Estimator} methods, if there is no state where the condition to switch is met, then we force-switch to next policy when the robot is within 1cm of the corresponding artifact.% e2e
% [0.95834 0.92776 0.902  ]
% [0.00494473 0.00441479 0.01344619]
% 106 46 94 246


% [0.46104 0.7821  0.7946  0.82184 0.83734 0.82776] [0.01048286 0.01384789 0.00930011 0.01266074 0.01296528 0.00892829]

% np.array([0.8544, 0.8284, 0.7160])

% 0.4610  0.4271 & 0.1012\\
%          On detection  & 0.7821 &  0.7560 & 0.6012\\
%          Q table & 0.7946 &  0.76356  & 0.5908 \\
%          CoM over feet  &  0.8218 & 0.7914 & 0.6680\\
%          Our RoA estimator & \textbf{0.8530} & \textbf{0.8247} & \textbf{0.7148} \\   
%          \hline
%          End to end  & - &  - & -\\
%          DQN  & \textbf{0.86428} & \textbf{0.83218} & \textbf{0.7240}\\
%          \hline

% \begin{table}[]
%     \centering
%     \begin{tabular}{c|c|c|c}
%     % \begin{tabular}{p{3cm}|x{1cm}|x{1cm}|x{1cm}}
%         %\hline
%         %\multicolumn{4}{c}{Artifact Type When Failure Occurs}\\
%         \hline
%          Switch method & Gaps & Jumps & Stairs\\   
%          \hline
%          Random  & 70.6 & 11.6 & 7.6  \\
%          On detection  & 21.4 & 3.3 & 15.2 \\
%          Lookup table  &  21.2 & 4.7 & 14.9 \\
%          CoM over feet  &  17.6 & 2.7 & 12.9 \\
%          Ours & 16.7 & 2.4 & 9.4\\
%          \hline
%          *DQN &  15.1 & 3.7 & 8.8  \\
%          *End to end & 4.2 & 1.8 & 3.7  \\
%         \hline
%     \end{tabular}
%     \caption{The artifact the robot was over when failure occurs, as a total percentage of all failures.\\ *Trained on the test domain (combinations of terrain types).}
%     \label{tab:failures}
% \end{table}

\begin{table}[]
    \vspace{3mm}
    \centering
    \begin{tabular}{c|c|c|c|c|c}
         %\hline
         %\multicolumn{3}{c}{Results of 2500 Trials on a Multi Terrain World}\\
         \hline
         Switch Method & \scriptsize{\% Total Dist.} & \scriptsize{\% Success} & \scriptsize{\% Gap Fail} & \scriptsize{\% Jump Fail} & \scriptsize{\% Stair Fail}\\   
         \hline
         Random  & 42.7 & 10.1 & 70.6 & 11.6 & \textbf{7.6} \\
         On detection  &   75.6 & 60.1 & 21.4 & 3.3 & 15.2 \\
         Lookup table &   76.3  & 59.0  &  21.2 & 4.7 & 14.9\\
         CoM over feet  & 79.1 & 66.8 &  17.6 & 2.7 & 12.9 \\
         Ours & \textbf{82.4} & \textbf{71.4} & \textbf{16.7} & \textbf{2.4} & 9.4\\   
         Ours no overlap& 17.5 & 0.7 &  58.6 & 12.9 & 27.7 \\   
         \hline
         *DQN  &  83.2 & 72.4 &  15.1 & 3.7 & 8.8  \\
         *End-to-end  &  \textbf{92.7} & \textbf{90.2} & \textbf{4.2} & \textbf{1.8} & \textbf{3.7}\\
         \hline
    \end{tabular}
    \caption{Results of each switching method on multi-terrain test worlds (2500 trials). The \% of the total distance covered, and the success rate for the robot reaching the end of the trial is shown. The final three columns show the \% of failures for each artifact type.\\ *Trained on the test domain (combinations of terrain types).}
    \label{tab:test_results}
\end{table}


% \begin{table}[]
%     \centering
%     \begin{tabular}{c|c|c}
%          \hline
%          \multicolumn{3}{c}{Results of 2500 Trials on a Multi Terrain World}\\
%          \hline
%          Switch Method & Percentage of Total Distance & Success Rate\\   
%          \hline
%          Our switch estimator & \textbf{0.8247} & \textbf{0.7148} \\   
%          \hline
%          End to end  &  \textbf{0.92776} & \textbf{0.9020}\\
%          DQN  &  0.8322 & 0.7240\\
%          \hline
%     \end{tabular}
%     \caption{Results from 2500 trials on a random test world for each switching method. We record the percentage of the total distance reached, and the success rate for the robot reaching the end of the trial.}    \label{tab:test_e2e_results}
% \end{table}


Table~\ref{tab:test_results} shows the results for multi-terrain test worlds. For less dynamic platforms it may be possible to switch controllers at any time after obstacle detection, however that was not the case for our scenarios: random switching performed the worst as expected with only 10.1\% success rate. Switching as soon as an artifact is detected does better than randomly switching with 60.1\% success, we suggest this is because switching early might give the policies enough time to align to an artifact. Fig.~\ref{fig:estimator}.b) shows it is preferential to switch early for some policies. \textbf{Lookup table} method performed similarly to the \textbf{On Detection} method. \textbf{CoM over feet} method performed relatively well with 66.8\% success. An advantage of this method is that it does not require further data collection once individual policies are trained, providing insight into where RoA overlap occurs for most policies.  \textbf{Our} switching method was the most robust, whilst following our condition that we only have access to each individual terrain artifact at training time, traversing 82.4\% of the terrain and reaching the final zone in 71.4\% of trials. Finally, we show the effect of training policies without considering RoA overlap. \textbf{Ours no overlap} performed poorly, Fig.~\ref{fig:test_results} shows that if trained without explicit state overlap, our policies are unable to successfully complete the multi terrain test environment. This result highlights the importance of RoA consideration when training dynamic policies where switching between controllers may be required.

Fig.~\ref{fig:plot} shows a single trial of the test world using our method. We can see the switch estimator predictions for each policy in the top figure, and the times our predictions prevented early switching (vertical green lines show detection, vertical red lines show when switching occurs). We can also see in the bottom plot the times that the CoM is over the feet, and instances our estimator switched outside of these regions ($\text{timestep}\approx875$).

The final three columns of Table~\ref{tab:test_results} shows the failure distribution of each switch method. We record where the robot was when failure occurs, given as a percentage of all trials. For each method, the most failures happened after switching to the Gaps policy. For instance, it contributed to to 16.7\% of a total (28.6\%) failures for our switching method. For all terrain types, these results show less failures than the single terrain experiments reported in Table~\ref{tab:individual_results}. This suggests we are improving the robustness of each policy using our switch estimator.

% This provides insight into where our system requires more robust policies, and more reliable swic

% This is in contrast to the results reported in Table~\ref{tab:individual_results}, where the Stairs policy was the least reliable. 

% We believe that this is because in the single artifact type case, the Stairs policy does not get a chance to stabilise for the upcoming Stairs artifact, whereas in the multi artifact type case, the flat portion of the following non-Stair artifact allows the robot to stabilise.

%We believe that after a  segment of stairs in the test conditions, the flat portion of the following non-stair artifact allows the robot to stabilise.

% Table.~\ref{tab:individual_results} shows the gaps policy on a single terrain has a failure rate of 39.6\%, indicating that our switch estimator 

% This is in contrast to the results in table.~\ref{tab:individual_results} where the stair controller was the least stable

% Performance improvements for each policy are consistent with the results from Table.~\ref{tab:test_results}, though interestingly do not match the baseline performances from table.~\ref{tab:individual_results}. This information can potentially be used to improve particular policies, and if necessary look at specific regions where new policies are required.

% \begin{table}[]
%     \centering
%     \begin{tabular}{c|c|c|c|c}
%         \hline
%         \multicolumn{5}{c}{Artifact Failure Count}\\
%         \hline
%          Switch method & Gaps & Jumps & Stairs & Total\\   
%          \hline
%          Random switching  & 1759 & 289 & 190 & 2238 \\
%          On detection  & 535 & 82 & 380 & 997\\
%          Look up table  &  529 & 118 & 372 & 1019\\
%          CoM over feet  &  441 & 67 & 323 & 831\\
%          Our switch estimator & 416 & 60 & 235 & 711\\
%          \hline
%          End to end & 106 & 46 & 94 & 246 \\
%          DQN &  377 & 92 & 221 &  690\\
%         \hline
%     \end{tabular}
%     \caption{A record of the artifact the robot was over when failure occurs for each switching method.}
%     \label{tab:failures}
% \end{table}


% 0.706429490616622	0.116064879356568	0.07630563002681
% 0.214	0.0328	0.152
% 0.212430618253189	0.047385279685967	0.149384102060844
% 0.176187725631769	0.026767749699158	0.129044524669073
% 0.166868073136428	0.024067510548523	0.094264416315049
% #DIV/0!	#DIV/0!	#DIV/0!
% 0.042227642276423	0.018325203252033	0.037447154471545
% 0.1508	0.0368	0.0884

%  Switch method & Gaps & Jumps & Stairs\\   
%  \hline
%  Random switching  & 0.7064 & 0.1161 & 0.0763  \\
%  On detection  & 0.2140 & 0.0328 & 0.1520 \\
%  Look up table  &  0.2124 & 0.0474 & 0.1494 \\
%  CoM over feet  &  0.1762 & 0.02677 & 0.1290 \\
%  Our switch estimator & 0.1669 & 0.0241 & 0.0943\\
%  \hline
%  *DQN &  0.1508 & 0.0368 & 0.0884  \\
%  *End to end & 0.0422 & 0.0183 & 0.0374  \\

% \begin{table}[]
%     \centering
%     \begin{tabular}{c|c|c|c}
%     % \begin{tabular}{p{3cm}|x{1cm}|x{1cm}|x{1cm}}
%         %\hline
%         %\multicolumn{4}{c}{Artifact Type When Failure Occurs}\\
%         \hline
%          Switch method & Gaps & Jumps & Stairs\\   
%          \hline
%          Random  & 70.6 & 11.6 & 7.6  \\
%          On detection  & 21.4 & 3.3 & 15.2 \\
%          Lookup table  &  21.2 & 4.7 & 14.9 \\
%          CoM over feet  &  17.6 & 2.7 & 12.9 \\
%          Ours & 16.7 & 2.4 & 9.4\\
%          \hline
%          *DQN &  15.1 & 3.7 & 8.8  \\
%          *End to end & 4.2 & 1.8 & 3.7  \\
%         \hline
%     \end{tabular}
%     \caption{The artifact the robot was over when failure occurs, as a total percentage of all failures.\\ *Trained on the test domain (combinations of terrain types).}
%     \label{tab:failures}
% \end{table}

\subsection{Comparison with training on multiple artifact terrains}
\label{sec:comparison}

For completeness, we also look at other methods that involve training on a full combination of terrain artifacts, including training a \textbf{Deep Q Network (DQN)} using our pre-trained policies, and a single \textbf{end-to-end policy}. Results are displayed in the last two rows of Table.~\ref{tab:test_results}. The \textbf{DQN} was provided with the artifact detection in the form of a one hot encoding appended to the robot state, and received the same reward as each policy, with an additional reward provided by our oracle terrain detector. We note that without the additional reward provided by the oracle the \textbf{DQN} failed to learn. For the \textbf{end-to-end} learning method, we applied the same reward and curriculum learning approach (from~\cite{tidd_guided_2020}) as our policies. Robot state + heightmap is provided as input, and torques are generated at the output. We note that without the curriculum the \textbf{end-to-end} method failed to learn.

Our estimator performs similarly to the \textbf{DQN} despite not seeing more than one terrain artifact type during training (71.4\% success compared to 72.4\%). While learning was substantially longer for the \textbf{end-to-end} policy (approx. 3 times longer than an individual policy), it performed the best with 90.2\% success rate. While these methods trained on the test domain perform well, it may not be possible to train on all expected terrain conditions on a real platform, where training policies separately allows us to refine each policy in a constrained setting. Furthermore, our method can include new behaviours as they become available, where the \textbf{DQN} and \textbf{end-to-end} methods fail when a new terrain is introduced.

We consider the occasion when a new terrain is introduced to an existing control suite. With our method, we train a policy for the new terrain artifact, and its switch estimator. Both the \textbf{end-to-end} policy, and the \textbf{DQN} method require retraining with all terrain conditions. Table~\ref{tab:re_training} shows the wall clock training time for all 3 methods when a new terrain is introduced. \textbf{TODO:} make sure $\pi_i$ is the default flat policy only

\begin{table}[]
    \vspace{3mm}
    \centering
    \begin{tabular}{c|c|c}
         \hline
         \scriptsize{\textbf{DQN (hrs)}} & \scriptsize{\textbf{end-to-end (hrs)}} & \scriptsize{\textbf{Ours (hrs)}}\\   
         \hline
         70.6 & 11.6 & \textbf{7.6} \\
         \hline
    \end{tabular}
    \caption{Wall clock time for retraining when a new terrain is introduced. Note: \textbf{end-to-end} and \textbf{DQN} require all terrains for retraining, \textbf{Ours} only requires the new terrain. Each method is trained with the same number of CPU cores.}
    \label{tab:re_training}
\end{table}

% \begin{figure}[tb!]
% \centering
% \subfloat[]{%
% \includegraphics[width=0.5\columnwidth]{images/plot_alive.png}}
% \hfill
% \subfloat[]{%
% \includegraphics[width=0.5\columnwidth]{images/plot_distance.png}}\hfill
% \hfill
% \subfloat[]{%
% \includegraphics[width=0.5\columnwidth]{images/plot_success.png}}\hfill
% \caption{Graphical representation of Table.~\ref{tab:test_results} including the standard deviation from the 5 random seeds. a) Shows the portion of time alive compared to the total possible time for a given trial, b) is the portion of distance covered, and c) is the success rate for reaching the end of a trial sequence.}
% \label{fig:test_results}
% \vspace{-3mm}
% \end{figure}



\begin{figure}[tb!]
\vspace{2mm}
\centering
\includegraphics[width=0.95\columnwidth]{images/plot.png}
\caption{Our method on a single trial in the test world. The top figure shows the switch estimate from the time the next artifact is detected until the robot has past the artifact. The bottom figure shows the terrain (pink) with foot (blue and green) and CoM height (red) when the CoM is over the stance foot. Green vertical lines indicate when the terrain was detected, red vertical lines show when switching occurred.}
\label{fig:plot}
% \vspace{-3mm}
\end{figure}

% \begin{figure}[tb!]
% \centering
% \includegraphics[width=1.0\columnwidth]{images/main_pic.png}
% % \caption{We pre-train policies for several artifact types including jumps, gaps and stairs, ensuring an Regions of Attraction (RoA) overlap for each policy. As a new terrain type is detected, we switch policies when the robot is in a state that is in the RoA for the next policy.}
% \caption{We design policies for each complex terrain type separately, ensuring common regions of the state between policies. Switching in these common regions results in desirable behaviour from the switched policy. To successfully switch between policies we train a switch estimator for each policy that learns when best to switch. Our method involves training on each artifact type separately, where training on multiple artifact types at once may be unavailable or dangerous.}
% \label{fig:plot}
% \vspace{-3mm}
% \end{figure}

% \caption{Our method on a single trial in the test world. The top figure shows the switch estimate from the time the next artifact is detected until the robot has past the artifact. The middle plot is the current policy being deployed, and when the switching occurs to the next policy. The bottom figure shows the terrain with foot and CoM height when the CoM is over the stance foot.}


% \begin{table}[]
%     \centering
%     \begin{tabular}{c|c|c|c}
%         \hline
%          & Time Alive & Distance & Success \\   
%          \hline
%          End to end  & 0.5249 &  0.4933 & 0.24\\
%          DQN  & 0.86428 & 0.83218 & 0.7240\\
         
%          \hline
%     \end{tabular}
%     \caption{Caption}
%     \label{tab:other_results}
% \end{table}

% \begin{figure}[tb!]
% \centering
% \includegraphics[width=1.0\columnwidth]{images/gaps_q_table.png}
% \caption{}
% \label{fig:q_table}
% \vspace{-3mm}
% \end{figure}



% Results summary:
% \begin{itemize}
%     \item TODO: Way to show that subpolicies have regions of attractions that overlap:
%     \begin{itemize}
%         \item Train subpolicies without controller overlap: no expert in reward, no expert cur?
%         \item Evaluate individual policies
%         \item Run baseline
%     \end{itemize}
%     \item Evaluate individual policies, 
%     \item Evaluate likelihoods for sections: graphics
%     \item Evaluate switching at given step
%     \item Evaluate success criteria
%     \item compare baseline, switching, and ours
% \end{itemize}
% Notes:
% \begin{itemize}
%     \item Compare the amount of information needed to switch: 
%     \begin{itemize}
%         \item none (switch as soon as artifact detected)
%         \item Randomly switch after an artifact detected
%         \item Switch based on distance since artifact detected
%         \item Mine: switch when configuration good: i.e. roa estimate
        
%     \end{itemize}
%     \item Histogram for each
%     \item Look at simple things like when is switching good between the methods: when foot is down (left foot over right?), where is the com. Any patterns. feature engineering: wider vs deeper. 
%     \item Other things to consider: training time (samples). Compare how good each method is on the training domain compared to the test..
%     \item success criteria may effect all results, evaluate some of these.
% \end{itemize}


% What plots should I have?

% Subpolicy results

% Results of individual experiments. Pics of 


% We evaluate our switching method on a test world. The test world is a random sequence of 7 terrain artifacts, with a distance of around 19m and dimensions drawn from the same uniform distributions as the training examples. Each test is performed 100 times, equating to 700 interactions with artifacts. The results are shown in table~\ref{tab:results}. 

% We compare our switching method to several benchmarks, with a baseline of switching controllers as soon as the robot's perception detects the next artifact. We try switching when the feet are close together and the centre of mass is over the feet. 

% After each run we record how long the robot has been alive out of a possible 3000 timesteps, how far the robot has walked out of the total terrain distance, and if the robot has successfully made it to the final flat area at the end of the terrain sequence.

% We evaluate several thresholds for success criteria.



